Learning Combinatorial Optimization on Graphs: A Survey with Applications to Networking

Existing approaches to solving combinatorial optimization problems on graphs suffer from the need to engineer each problem algorithmically, with practical problems recurring in many instances. The practical side of theoretical computer science, such as computational complexity, then needs to be addressed. Relevant developments in machine learning research on graphs are surveyed for this purpose. We organize and compare the structures involved with learning to solve combinatorial optimization problems, with a special eye on the telecommunications domain and its continuous development of live and research networks.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> IEEEtran/tools/README <==

August 26, 2015


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. The \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later.

 3. The \IEEEnoauxwrite command.

 4. The IEEE itemize, enumerate and description list environments.

 5. The complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 6. The \IEEEQEDhere and \IEEEQEDhereams commands to provide amsthm.sty
    \qedhere functionality to IEEEproof. \IEEEQEDhere is for simple use
    "right on the spot" such as within an IEEEeqnarry:

    \begin{IEEEproof}
       \begin{IEEEeqnarray}{rCl+x*}
        x & = & y & \nonumber\IEEEQEDhere
       \end{IEEEeqnarray}
    \end{IEEEproof}

    While \IEEEQEDhereams is like amsthm's venerable \qedhere and is
    for use within the standard equation environment:

    \begin{IEEEproof}
     \begin{equation}
       x = y \nonumber\IEEEQEDhereams\quad
     \end{equation}
    \end{IEEEproof}

    Note that the qedhere style is normally not done with IEEE-related
    work so these are undocumented features of IEEEtran.cls.

    Thanks Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser for
    suggesting this feature.



IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
2015/08/26 V1.5 (V1.8b of IEEEtran.cls) changes:

 1) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 2) Fix bug with IEEEeqnarray equation number foreground color
    under the color environment of Beamer class.
    Thanks to Joschi Brauchle for reporting this problem.

 3) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.



********************************** Files **********************************

README                - This file.

changelog.txt         - The revision history.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> spotcolor/spotcolorhks.tex <==
\NewSpotColorSpace{HKS}
\AddSpotColor {HKS} {HKS05N} {HKS\SpotSpace 05\SpotSpace N} {0.0 0.15 1.0 0.0}
\AddSpotColor {HKS} {HKS14N} {HKS\SpotSpace 14\SpotSpace N} {0.0 0.75 0.7 0.0}
\AddSpotColor {HKS} {HKS17N} {HKS\SpotSpace 17\SpotSpace N} {1.0 0.1 0.6 0.0}
\AddSpotColor {HKS} {HKS24N} {HKS\SpotSpace 24\SpotSpace N} {0.0 0.1 0.3 0.0}
\AddSpotColor {HKS} {HKS38N} {HKS\SpotSpace 38\SpotSpace N} {0.9 0.5 0.15 0.3}
\AddSpotColor {HKS} {HKS49N} {HKS\SpotSpace 49\SpotSpace N} {1.0 0.0 0.08 0.0}
\AddSpotColor {HKS} {HKS57N} {HKS\SpotSpace 57\SpotSpace N} {0.8 0.0 0.6 0.7}
\AddSpotColor {HKS} {HKS68N} {HKS\SpotSpace 68\SpotSpace N} {0.2 0.07 1.0 0.0}
\AddSpotColor {HKS} {HKS74N} {HKS\SpotSpace 74\SpotSpace N} {0.0 0.3 1.0 0.25}
\AddSpotColor {HKS} {HKS92N} {HKS\SpotSpace 92\SpotSpace N} {0.1 0.0 0.1 0.5}


==> spotcolor/spotcolorpantone.tex <==
\NewSpotColorSpace{PANTONE}
\AddSpotColor{PANTONE} {PANTONE100PC} {PANTONE\SpotSpace 100\SpotSpace PC} {0 0 0.51 0}
\AddSpotColor{PANTONE} {PANTONE101PC} {PANTONE\SpotSpace 101\SpotSpace PC} {0 0 0.79 0}
\AddSpotColor{PANTONE} {PANTONE102PC} {PANTONE\SpotSpace 102\SpotSpace PC} {0 0 0.95 0}
\AddSpotColor{PANTONE} {PANTONE103PC} {PANTONE\SpotSpace 103\SpotSpace PC} {0 0.03 1 0.18}
\AddSpotColor{PANTONE} {PANTONE104PC} {PANTONE\SpotSpace 104\SpotSpace PC} {0 0.03 1 0.3}
\AddSpotColor{PANTONE} {PANTONE105PC} {PANTONE\SpotSpace 105\SpotSpace PC} {0 0.03 1 0.5}
\AddSpotColor{PANTONE} {PANTONE106PC} {PANTONE\SpotSpace 106\SpotSpace PC} {0 0.02 0.69 0}
\AddSpotColor{PANTONE} {PANTONE107PC} {PANTONE\SpotSpace 107\SpotSpace PC} {0 0.04 0.79 0}
\AddSpotColor{PANTONE} {PANTONE108PC} {PANTONE\SpotSpace 108\SpotSpace PC} {0 0.06 0.95 0}
\AddSpotColor{PANTONE} {PANTONE109PC} {PANTONE\SpotSpace 109\SpotSpace PC} {0 0.1 1 0}
\AddSpotColor{PANTONE} {PANTONE110PC} {PANTONE\SpotSpace 110\SpotSpace PC} {0 0.12 1 0.07}
\AddSpotColor{PANTONE} {PANTONE111PC} {PANTONE\SpotSpace 111\SpotSpace PC} {0 0.11 1 0.27}
\AddSpotColor{PANTONE} {PANTONE112PC} {PANTONE\SpotSpace 112\SpotSpace PC} {0 0.1 1 0.38}
\AddSpotColor{PANTONE} {PANTONE113PC} {PANTONE\SpotSpace 113\SpotSpace PC} {0 0.07 0.66 0}
\AddSpotColor{PANTONE} {PANTONE114PC} {PANTONE\SpotSpace 114\SpotSpace PC} {0 0.08 0.73 0}
\AddSpotColor{PANTONE} {PANTONE115PC} {PANTONE\SpotSpace 115\SpotSpace PC} {0 0.09 0.8 0}
\AddSpotColor{PANTONE} {PANTONE116PC} {PANTONE\SpotSpace 116\SpotSpace PC} {0 0.16 1 0}
\AddSpotColor{PANTONE} {PANTONE117PC} {PANTONE\SpotSpace 117\SpotSpace PC} {0 0.18 1 0.15}
\AddSpotColor{PANTONE} {PANTONE118PC} {PANTONE\SpotSpace 118\SpotSpace PC} {0 0.18 1 0.27}
\AddSpotColor{PANTONE} {PANTONE119PC} {PANTONE\SpotSpace 119\SpotSpace PC} {0 0.12 1 0.49}
\AddSpotColor{PANTONE} {PANTONE120PC} {PANTONE\SpotSpace 120\SpotSpace PC} {0 0.09 0.58 0}
\AddSpotColor{PANTONE} {PANTONE121PC} {PANTONE\SpotSpace 121\SpotSpace PC} {0 0.11 0.69 0}
\AddSpotColor{PANTONE} {PANTONE122PC} {PANTONE\SpotSpace 122\SpotSpace PC} {0 0.17 0.8 0}
\AddSpotColor{PANTONE} {PANTONE123PC} {PANTONE\SpotSpace 123\SpotSpace PC} {0 0.24 0.94 0}
\AddSpotColor{PANTONE} {PANTONE124PC} {PANTONE\SpotSpace 124\SpotSpace PC} {0 0.28 1 0.06}
\AddSpotColor{PANTONE} {PANTONE125PC} {PANTONE\SpotSpace 125\SpotSpace PC} {0 0.26 1 0.26}
\AddSpotColor{PANTONE} {PANTONE126PC} {PANTONE\SpotSpace 126\SpotSpace PC} {0 0.25 1 0.37}
\AddSpotColor{PANTONE} {PANTONE127PC} {PANTONE\SpotSpace 127\SpotSpace PC} {0 0.07 0.5 0}
\AddSpotColor{PANTONE} {PANTONE128PC} {PANTONE\SpotSpace 128\SpotSpace PC} {0 0.11 0.65 0}
\AddSpotColor{PANTONE} {PANTONE129PC} {PANTONE\SpotSpace 129\SpotSpace PC} {0 0.16 0.77 0}
\AddSpotColor{PANTONE} {PANTONE130PC} {PANTONE\SpotSpace 130\SpotSpace PC} {0 0.3 1 0}
\AddSpotColor{PANTONE} {PANTONE131PC} {PANTONE\SpotSpace 131\SpotSpace PC} {0 0.32 1 0.09}
\AddSpotColor{PANTONE} {PANTONE132PC} {PANTONE\SpotSpace 132\SpotSpace PC} {0 0.28 1 0.3}
\AddSpotColor{PANTONE} {PANTONE133PC} {PANTONE\SpotSpace 133\SpotSpace PC} {0 0.2 1 0.56}
\AddSpotColor{PANTONE} {PANTONE134PC} {PANTONE\SpotSpace 134\SpotSpace PC} {0 0.11 0.45 0}
\AddSpotColor{PANTONE} {PANTONE135PC} {PANTONE\SpotSpace 135\SpotSpace PC} {0 0.19 0.6 0}
\AddSpotColor{PANTONE} {PANTONE136PC} {PANTONE\SpotSpace 136\SpotSpace PC} {0 0.27 0.76 0}
\AddSpotColor{PANTONE} {PANTONE137PC} {PANTONE\SpotSpace 137\SpotSpace PC} {0 0.35 0.9 0}
\AddSpotColor{PANTONE} {PANTONE138PC} {PANTONE\SpotSpace 138\SpotSpace PC} {0 0.42 1 0.01}
\AddSpotColor{PANTONE} {PANTONE139PC} {PANTONE\SpotSpace 139\SpotSpace PC} {0 0.37 1 0.23}
\AddSpotColor{PANTONE} {PANTONE140PC} {PANTONE\SpotSpace 140\SpotSpace PC} {0 0.27 1 0.54}
\AddSpotColor{PANTONE} {PANTONE141PC} {PANTONE\SpotSpace 141\SpotSpace PC} {0 0.19 0.51 0}
\AddSpotColor{PANTONE} {PANTONE142PC} {PANTONE\SpotSpace 142\SpotSpace PC} {0 0.28 0.76 0}
\AddSpotColor{PANTONE} {PANTONE143PC} {PANTONE\SpotSpace 143\SpotSpace PC} {0 0.35 0.85 0}
\AddSpotColor{PANTONE} {PANTONE144PC} {PANTONE\SpotSpace 144\SpotSpace PC} {0 0.48 1 0}
\AddSpotColor{PANTONE} {PANTONE145PC} {PANTONE\SpotSpace 145\SpotSpace PC} {0 0.47 1 0.08}
\AddSpotColor{PANTONE} {PANTONE146PC} {PANTONE\SpotSpace 146\SpotSpace PC} {0 0.43 1 0.33}
\AddSpotColor{PANTONE} {PANTONE147PC} {PANTONE\SpotSpace 147\SpotSpace PC} {0 0.28 1 0.56}
\AddSpotColor{PANTONE} {PANTONE148PC} {PANTONE\SpotSpace 148\SpotSpace PC} {0 0.16 0.37 0}
\AddSpotColor{PANTONE} {PANTONE149PC} {PANTONE\SpotSpace 149\SpotSpace PC} {0 0.23 0.47 0}
\AddSpotColor{PANTONE} {PANTONE150PC} {PANTONE\SpotSpace 150\SpotSpace PC} {0 0.35 0.7 0}
\AddSpotColor{PANTONE} {PANTONE151PC} {PANTONE\SpotSpace 151\SpotSpace PC} {0 0.48 0.95 0}
\AddSpotColor{PANTONE} {PANTONE152PC} {PANTONE\SpotSpace 152\SpotSpace PC} {0 0.51 1 0.01}
\AddSpotColor{PANTONE} {PANTONE153PC} {PANTONE\SpotSpace 153\SpotSpace PC} {0 0.46 1 0.18}
\AddSpotColor{PANTONE} {PANTONE154PC} {PANTONE\SpotSpace 154\SpotSpace PC} {0 0.46 1 0.34}
\AddSpotColor{PANTONE} {PANTONE155PC} {PANTONE\SpotSpace 155\SpotSpace PC} {0 0.12 0.28 0}
\AddSpotColor{PANTONE} {PANTONE156PC} {PANTONE\SpotSpace 156\SpotSpace PC} {0 0.22 0.42 0}
\AddSpotColor{PANTONE} {PANTONE157PC} {PANTONE\SpotSpace 157\SpotSpace PC} {0 0.43 0.7 0}
\AddSpotColor{PANTONE} {PANTONE158PC} {PANTONE\SpotSpace 158\SpotSpace PC} {0 0.61 0.97 0}
\AddSpotColor{PANTONE} {PANTONE159PC} {PANTONE\SpotSpace 159\SpotSpace PC} {0 0.66 1 0.07}
\AddSpotColor{PANTONE} {PANTONE160PC} {PANTONE\SpotSpace 160\SpotSpace PC} {0 0.62 1 0.32}
\AddSpotColor{PANTONE} {PANTONE161PC} {PANTONE\SpotSpace 161\SpotSpace PC} {0 0.52 1 0.64}
\AddSpotColor{PANTONE} {PANTONE162PC} {PANTONE\SpotSpace 162\SpotSpace PC} {0 0.15 0.22 0}
\AddSpotColor{PANTONE} {PANTONE163PC} {PANTONE\SpotSpace 163\SpotSpace PC} {0 0.31 0.44 0}
\AddSpotColor{PANTONE} {PANTONE164PC} {PANTONE\SpotSpace 164\SpotSpace PC} {0 0.46 0.73 0}
\AddSpotColor{PANTONE} {PANTONE165PC} {PANTONE\SpotSpace 165\SpotSpace PC} {0 0.59 0.96 0}
\AddSpotColor{PANTONE} {PANTONE166PC} {PANTONE\SpotSpace 166\SpotSpace PC} {0 0.64 1 0}
\AddSpotColor{PANTONE} {PANTONE167PC} {PANTONE\SpotSpace 167\SpotSpace PC} {0 0.6 1 0.17}
\AddSpotColor{PANTONE} {PANTONE168PC} {PANTONE\SpotSpace 168\SpotSpace PC} {0 0.57 1 0.59}
\AddSpotColor{PANTONE} {PANTONE169PC} {PANTONE\SpotSpace 169\SpotSpace PC} {0 0.2 0.2 0}
\AddSpotColor{PANTONE} {PANTONE170PC} {PANTONE\SpotSpace 170\SpotSpace PC} {0 0.4 0.44 0}
\AddSpotColor{PANTONE} {PANTONE171PC} {PANTONE\SpotSpace 171\SpotSpace PC} {0 0.53 0.68 0}
\AddSpotColor{PANTONE} {PANTONE172PC} {PANTONE\SpotSpace 172\SpotSpace PC} {0 0.66 0.88 0}
\AddSpotColor{PANTONE} {PANTONE173PC} {PANTONE\SpotSpace 173\SpotSpace PC} {0 0.69 1 0.04}
\AddSpotColor{PANTONE} {PANTONE174PC} {PANTONE\SpotSpace 174\SpotSpace PC} {0 0.7 1 0.36}
\AddSpotColor{PANTONE} {PANTONE175PC} {PANTONE\SpotSpace 175\SpotSpace PC} {0 0.65 1 0.6}
\AddSpotColor{PANTONE} {PANTONE176PC} {PANTONE\SpotSpace 176\SpotSpace PC} {0 0.25 0.18 0}
\AddSpotColor{PANTONE} {PANTONE177PC} {PANTONE\SpotSpace 177\SpotSpace PC} {0 0.45 0.4 0}
\AddSpotColor{PANTONE} {PANTONE178PC} {PANTONE\SpotSpace 178\SpotSpace PC} {0 0.59 0.56 0}
\AddSpotColor{PANTONE} {PANTONE179PC} {PANTONE\SpotSpace 179\SpotSpace PC} {0 0.79 1 0}
\AddSpotColor{PANTONE} {PANTONE180PC} {PANTONE\SpotSpace 180\SpotSpace PC} {0 0.79 1 0.11}
\AddSpotColor{PANTONE} {PANTONE181PC} {PANTONE\SpotSpace 181\SpotSpace PC} {0 0.74 1 0.47}
\AddSpotColor{PANTONE} {PANTONE182PC} {PANTONE\SpotSpace 182\SpotSpace PC} {0 0.26 0.1 0}
\AddSpotColor{PANTONE} {PANTONE183PC} {PANTONE\SpotSpace 183\SpotSpace PC} {0 0.46 0.21 0}
\AddSpotColor{PANTONE} {PANTONE184PC} {PANTONE\SpotSpace 184\SpotSpace PC} {0 0.68 0.41 0}
\AddSpotColor{PANTONE} {PANTONE185PC} {PANTONE\SpotSpace 185\SpotSpace PC} {0 0.91 0.76 0}
\AddSpotColor{PANTONE} {PANTONE186PC} {PANTONE\SpotSpace 186\SpotSpace PC} {0 1 0.81 0.04}
\AddSpotColor{PANTONE} {PANTONE187PC} {PANTONE\SpotSpace 187\SpotSpace PC} {0 1 0.79 0.2}
\AddSpotColor{PANTONE} {PANTONE188PC} {PANTONE\SpotSpace 188\SpotSpace PC} {0 0.97 1 0.5}
\AddSpotColor{PANTONE} {PANTONE189PC} {PANTONE\SpotSpace 189\SpotSpace PC} {0 0.37 0.1 0}
\AddSpotColor{PANTONE} {PANTONE190PC} {PANTONE\SpotSpace 190\SpotSpace PC} {0 0.55 0.22 0}
\AddSpotColor{PANTONE} {PANTONE191PC} {PANTONE\SpotSpace 191\SpotSpace PC} {0 0.76 0.38 0}
\AddSpotColor{PANTONE} {PANTONE192PC} {PANTONE\SpotSpace 192\SpotSpace PC} {0 1 0.68 0}
\AddSpotColor{PANTONE} {PANTONE193PC} {PANTONE\SpotSpace 193\SpotSpace PC} {0 1 0.66 0.13}
\AddSpotColor{PANTONE} {PANTONE194PC} {PANTONE\SpotSpace 194\SpotSpace PC} {0 1 0.64 0.33}
\AddSpotColor{PANTONE} {PANTONE195PC} {PANTONE\SpotSpace 195\SpotSpace PC} {0 1 0.6 0.55}
\AddSpotColor{PANTONE} {PANTONE196PC} {PANTONE\SpotSpace 196\SpotSpace PC} {0 0.25 0.04 0}
\AddSpotColor{PANTONE} {PANTONE197PC} {PANTONE\SpotSpace 197\SpotSpace PC} {0 0.45 0.1 0}
\AddSpotColor{PANTONE} {PANTONE198PC} {PANTONE\SpotSpace 198\SpotSpace PC} {0 0.78 0.33 0}
\AddSpotColor{PANTONE} {PANTONE199PC} {PANTONE\SpotSpace 199\SpotSpace PC} {0 1 0.62 0}
\AddSpotColor{PANTONE} {PANTONE200PC} {PANTONE\SpotSpace 200\SpotSpace PC} {0 1 0.63 0.12}
\AddSpotColor{PANTONE} {PANTONE201PC} {PANTONE\SpotSpace 201\SpotSpace PC} {0 1 0.63 0.29}
\AddSpotColor{PANTONE} {PANTONE202PC} {PANTONE\SpotSpace 202\SpotSpace PC} {0 1 0.61 0.43}
\AddSpotColor{PANTONE} {PANTONE203PC} {PANTONE\SpotSpace 203\SpotSpace PC} {0 0.34 0.03 0}
\AddSpotColor{PANTONE} {PANTONE204PC} {PANTONE\SpotSpace 204\SpotSpace PC} {0 0.58 0.03 0}
\AddSpotColor{PANTONE} {PANTONE205PC} {PANTONE\SpotSpace 205\SpotSpace PC} {0 0.84 0.09 0}
\AddSpotColor{PANTONE} {PANTONE206PC} {PANTONE\SpotSpace 206\SpotSpace PC} {0 1 0.38 0.03}
\AddSpotColor{PANTONE} {PANTONE207PC} {PANTONE\SpotSpace 207\SpotSpace PC} {0 1 0.43 0.19}
\AddSpotColor{PANTONE} {PANTONE208PC} {PANTONE\SpotSpace 208\SpotSpace PC} {0 1 0.36 0.37}
\AddSpotColor{PANTONE} {PANTONE209PC} {PANTONE\SpotSpace 209\SpotSpace PC} {0 1 0.34 0.53}
\AddSpotColor{PANTONE} {PANTONE210PC} {PANTONE\SpotSpace 210\SpotSpace PC} {0 0.39 0.06 0}
\AddSpotColor{PANTONE} {PANTONE211PC} {PANTONE\SpotSpace 211\SpotSpace PC} {0 0.55 0.08 0}
\AddSpotColor{PANTONE} {PANTONE212PC} {PANTONE\SpotSpace 212\SpotSpace PC} {0 0.72 0.11 0}
\AddSpotColor{PANTONE} {PANTONE213PC} {PANTONE\SpotSpace 213\SpotSpace PC} {0 0.95 0.27 0}
\AddSpotColor{PANTONE} {PANTONE214PC} {PANTONE\SpotSpace 214\SpotSpace PC} {0 1 0.34 0.08}
\AddSpotColor{PANTONE} {PANTONE215PC} {PANTONE\SpotSpace 215\SpotSpace PC} {0 1 0.35 0.27}
\AddSpotColor{PANTONE} {PANTONE216PC} {PANTONE\SpotSpace 216\SpotSpace PC} {0 0.95 0.4 0.49}
\AddSpotColor{PANTONE} {PANTONE217PC} {PANTONE\SpotSpace 217\SpotSpace PC} {0 0.28 0 0}
\AddSpotColor{PANTONE} {PANTONE218PC} {PANTONE\SpotSpace 218\SpotSpace PC} {0.02 0.61 0 0}
\AddSpotColor{PANTONE} {PANTONE219PC} {PANTONE\SpotSpace 219\SpotSpace PC} {0.01 0.88 0 0}
\AddSpotColor{PANTONE} {PANTONE220PC} {PANTONE\SpotSpace 220\SpotSpace PC} {0 1 0.13 0.17}
\AddSpotColor{PANTONE} {PANTONE221PC} {PANTONE\SpotSpace 221\SpotSpace PC} {0 1 0.15 0.3}
\AddSpotColor{PANTONE} {PANTONE222PC} {PANTONE\SpotSpace 222\SpotSpace PC} {0 1 0.1 0.59}
\AddSpotColor{PANTONE} {PANTONE223PC} {PANTONE\SpotSpace 223\SpotSpace PC} {0 0.46 0 0}
\AddSpotColor{PANTONE} {PANTONE224PC} {PANTONE\SpotSpace 224\SpotSpace PC} {0.01 0.63 0 0}
\AddSpotColor{PANTONE} {PANTONE225PC} {PANTONE\SpotSpace 225\SpotSpace PC} {0.01 0.83 0 0}
\AddSpotColor{PANTONE} {PANTONE226PC} {PANTONE\SpotSpace 226\SpotSpace PC} {0 0.99 0 0}
\AddSpotColor{PANTONE} {PANTONE227PC} {PANTONE\SpotSpace 227\SpotSpace PC} {0 1 0.07 0.19}
\AddSpotColor{PANTONE} {PANTONE228PC} {PANTONE\SpotSpace 228\SpotSpace PC} {0 1 0.04 0.41}
\AddSpotColor{PANTONE} {PANTONE229PC} {PANTONE\SpotSpace 229\SpotSpace PC} {0 1 0.15 0.6}
\AddSpotColor{PANTONE} {PANTONE230PC} {PANTONE\SpotSpace 230\SpotSpace PC} {0 0.34 0 0}
\AddSpotColor{PANTONE} {PANTONE231PC} {PANTONE\SpotSpace 231\SpotSpace PC} {0.01 0.52 0 0}
\AddSpotColor{PANTONE} {PANTONE232PC} {PANTONE\SpotSpace 232\SpotSpace PC} {0.03 0.67 0 0}
\AddSpotColor{PANTONE} {PANTONE233PC} {PANTONE\SpotSpace 233\SpotSpace PC} {0.11 1 0 0}
\AddSpotColor{PANTONE} {PANTONE234PC} {PANTONE\SpotSpace 234\SpotSpace PC} {0.06 1 0 0.26}
\AddSpotColor{PANTONE} {PANTONE235PC} {PANTONE\SpotSpace 235\SpotSpace PC} {0.05 1 0 0.4}
\AddSpotColor{PANTONE} {PANTONE236PC} {PANTONE\SpotSpace 236\SpotSpace PC} {0.01 0.3 0 0}
\AddSpotColor{PANTONE} {PANTONE237PC} {PANTONE\SpotSpace 237\SpotSpace PC} {0.03 0.49 0 0}
\AddSpotColor{PANTONE} {PANTONE238PC} {PANTONE\SpotSpace 238\SpotSpace PC} {0.06 0.63 0 0}
\AddSpotColor{PANTONE} {PANTONE239PC} {PANTONE\SpotSpace 239\SpotSpace PC} {0.11 0.79 0 0}
\AddSpotColor{PANTONE} {PANTONE240PC} {PANTONE\SpotSpace 240\SpotSpace PC} {0.18 0.94 0 0}
\AddSpotColor{PANTONE} {PANTONE241PC} {PANTONE\SpotSpace 241\SpotSpace PC} {0.27 1 0 0.02}
\AddSpotColor{PANTONE} {PANTONE242PC} {PANTONE\SpotSpace 242\SpotSpace PC} {0.1 1 0 0.49}
\AddSpotColor{PANTONE} {PANTONE243PC} {PANTONE\SpotSpace 243\SpotSpace PC} {0.05 0.29 0 0}
\AddSpotColor{PANTONE} {PANTONE244PC} {PANTONE\SpotSpace 244\SpotSpace PC} {0.09 0.38 0 0}
\AddSpotColor{PANTONE} {PANTONE245PC} {PANTONE\SpotSpace 245\SpotSpace PC} {0.14 0.53 0 0}
\AddSpotColor{PANTONE} {PANTONE246PC} {PANTONE\SpotSpace 246\SpotSpace PC} {0.29 0.9 0 0}
\AddSpotColor{PANTONE} {PANTONE247PC} {PANTONE\SpotSpace 247\SpotSpace PC} {0.36 1 0 0}
\AddSpotColor{PANTONE} {PANTONE248PC} {PANTONE\SpotSpace 248\SpotSpace PC} {0.4 1 0 0.02}
\AddSpotColor{PANTONE} {PANTONE249PC} {PANTONE\SpotSpace 249\SpotSpace PC} {0.4 1 0 0.28}
\AddSpotColor{PANTONE} {PANTONE250PC} {PANTONE\SpotSpace 250\SpotSpace PC} {0.05 0.18 0 0}
\AddSpotColor{PANTONE} {PANTONE251PC} {PANTONE\SpotSpace 251\SpotSpace PC} {0.13 0.39 0 0}
\AddSpotColor{PANTONE} {PANTONE252PC} {PANTONE\SpotSpace 252\SpotSpace PC} {0.24 0.56 0 0}
\AddSpotColor{PANTONE} {PANTONE253PC} {PANTONE\SpotSpace 253\SpotSpace PC} {0.43 0.95 0 0}
\AddSpotColor{PANTONE} {PANTONE254PC} {PANTONE\SpotSpace 254\SpotSpace PC} {0.5 1 0 0}
\AddSpotColor{PANTONE} {PANTONE255PC} {PANTONE\SpotSpace 255\SpotSpace PC} {0.51 1 0 0.25}
\AddSpotColor{PANTONE} {PANTONE256PC} {PANTONE\SpotSpace 256\SpotSpace PC} {0.07 0.2 0 0}
\AddSpotColor{PANTONE} {PANTONE257PC} {PANTONE\SpotSpace 257\SpotSpace PC} {0.14 0.34 0 0}
\AddSpotColor{PANTONE} {PANTONE258PC} {PANTONE\SpotSpace 258\SpotSpace PC} {0.43 0.76 0 0}
\AddSpotColor{PANTONE} {PANTONE259PC} {PANTONE\SpotSpace 259\SpotSpace PC} {0.55 1 0 0.15}
\AddSpotColor{PANTONE} {PANTONE260PC} {PANTONE\SpotSpace 260\SpotSpace PC} {0.52 1 0 0.26}
\AddSpotColor{PANTONE} {PANTONE261PC} {PANTONE\SpotSpace 261\SpotSpace PC} {0.48 1 0 0.4}
\AddSpotColor{PANTONE} {PANTONE262PC} {PANTONE\SpotSpace 262\SpotSpace PC} {0.45 1 0 0.55}
\AddSpotColor{PANTONE} {PANTONE263PC} {PANTONE\SpotSpace 263\SpotSpace PC} {0.1 0.14 0 0}
\AddSpotColor{PANTONE} {PANTONE264PC} {PANTONE\SpotSpace 264\SpotSpace PC} {0.26 0.28 0 0}
\AddSpotColor{PANTONE} {PANTONE265PC} {PANTONE\SpotSpace 265\SpotSpace PC} {0.54 0.56 0 0}
\AddSpotColor{PANTONE} {PANTONE266PC} {PANTONE\SpotSpace 266\SpotSpace PC} {0.79 0.9 0 0}
\AddSpotColor{PANTONE} {PANTONE267PC} {PANTONE\SpotSpace 267\SpotSpace PC} {0.89 1 0 0}
\AddSpotColor{PANTONE} {PANTONE268PC} {PANTONE\SpotSpace 268\SpotSpace PC} {0.82 1 0 0.12}
\AddSpotColor{PANTONE} {PANTONE269PC} {PANTONE\SpotSpace 269\SpotSpace PC} {0.78 1 0 0.33}
\AddSpotColor{PANTONE} {PANTONE270PC} {PANTONE\SpotSpace 270\SpotSpace PC} {0.31 0.27 0 0}
\AddSpotColor{PANTONE} {PANTONE271PC} {PANTONE\SpotSpace 271\SpotSpace PC} {0.43 0.37 0 0}
\AddSpotColor{PANTONE} {PANTONE272PC} {PANTONE\SpotSpace 272\SpotSpace PC} {0.58 0.48 0 0}
\AddSpotColor{PANTONE} {PANTONE273PC} {PANTONE\SpotSpace 273\SpotSpace PC} {1 0.96 0 0.08}
\AddSpotColor{PANTONE} {PANTONE274PC} {PANTONE\SpotSpace 274\SpotSpace PC} {1 1 0 0.28}
\AddSpotColor{PANTONE} {PANTONE275PC} {PANTONE\SpotSpace 275\SpotSpace PC} {0.98 1 0 0.43}
\AddSpotColor{PANTONE} {PANTONE276PC} {PANTONE\SpotSpace 276\SpotSpace PC} {1 1 0 0.58}
\AddSpotColor{PANTONE} {PANTONE277PC} {PANTONE\SpotSpace 277\SpotSpace PC} {0.27 0.07 0 0}
\AddSpotColor{PANTONE} {PANTONE278PC} {PANTONE\SpotSpace 278\SpotSpace PC} {0.39 0.14 0 0}
\AddSpotColor{PANTONE} {PANTONE279PC} {PANTONE\SpotSpace 279\SpotSpace PC} {0.68 0.34 0 0}
\AddSpotColor{PANTONE} {PANTONE280PC} {PANTONE\SpotSpace 280\SpotSpace PC} {1 0.72 0 0.18}
\AddSpotColor{PANTONE} {PANTONE281PC} {PANTONE\SpotSpace 281\SpotSpace PC} {1 0.72 0 0.32}
\AddSpotColor{PANTONE} {PANTONE282PC} {PANTONE\SpotSpace 282\SpotSpace PC} {1 0.68 0 0.54}
\AddSpotColor{PANTONE} {PANTONE283PC} {PANTONE\SpotSpace 283\SpotSpace PC} {0.35 0.09 0 0}
\AddSpotColor{PANTONE} {PANTONE284PC} {PANTONE\SpotSpace 284\SpotSpace PC} {0.55 0.19 0 0}
\AddSpotColor{PANTONE} {PANTONE285PC} {PANTONE\SpotSpace 285\SpotSpace PC} {0.89 0.43 0 0}
\AddSpotColor{PANTONE} {PANTONE286PC} {PANTONE\SpotSpace 286\SpotSpace PC} {1 0.66 0 0.02}
\AddSpotColor{PANTONE} {PANTONE287PC} {PANTONE\SpotSpace 287\SpotSpace PC} {1 0.68 0 0.12}
\AddSpotColor{PANTONE} {PANTONE288PC} {PANTONE\SpotSpace 288\SpotSpace PC} {1 0.67 0 0.23}
\AddSpotColor{PANTONE} {PANTONE289PC} {PANTONE\SpotSpace 289\SpotSpace PC} {1 0.64 0 0.6}
\AddSpotColor{PANTONE} {PANTONE290PC} {PANTONE\SpotSpace 290\SpotSpace PC} {0.25 0.02 0 0}
\AddSpotColor{PANTONE} {PANTONE291PC} {PANTONE\SpotSpace 291\SpotSpace PC} {0.33 0.03 0 0}
\AddSpotColor{PANTONE} {PANTONE292PC} {PANTONE\SpotSpace 292\SpotSpace PC} {0.49 0.11 0 0}
\AddSpotColor{PANTONE} {PANTONE293PC} {PANTONE\SpotSpace 293\SpotSpace PC} {1 0.57 0 0.02}
\AddSpotColor{PANTONE} {PANTONE294PC} {PANTONE\SpotSpace 294\SpotSpace PC} {1 0.58 0 0.21}
\AddSpotColor{PANTONE} {PANTONE295PC} {PANTONE\SpotSpace 295\SpotSpace PC} {1 0.57 0 0.4}
\AddSpotColor{PANTONE} {PANTONE296PC} {PANTONE\SpotSpace 296\SpotSpace PC} {1 0.46 0 0.7}
\AddSpotColor{PANTONE} {PANTONE297PC} {PANTONE\SpotSpace 297\SpotSpace PC} {0.49 0.01 0 0}
\AddSpotColor{PANTONE} {PANTONE298PC} {PANTONE\SpotSpace 298\SpotSpace PC} {0.69 0.07 0 0}
\AddSpotColor{PANTONE} {PANTONE299PC} {PANTONE\SpotSpace 299\SpotSpace PC} {0.85 0.19 0 0}
\AddSpotColor{PANTONE} {PANTONE300PC} {PANTONE\SpotSpace 300\SpotSpace PC} {1 0.44 0 0}
\AddSpotColor{PANTONE} {PANTONE301PC} {PANTONE\SpotSpace 301\SpotSpace PC} {1 0.45 0 0.18}
\AddSpotColor{PANTONE} {PANTONE302PC} {PANTONE\SpotSpace 302\SpotSpace PC} {1 0.25 0 0.5}
\AddSpotColor{PANTONE} {PANTONE303PC} {PANTONE\SpotSpace 303\SpotSpace PC} {1 0.11 0 0.74}
\AddSpotColor{PANTONE} {PANTONE304PC} {PANTONE\SpotSpace 304\SpotSpace PC} {0.3 0 0.08 0}
\AddSpotColor{PANTONE} {PANTONE305PC} {PANTONE\SpotSpace 305\SpotSpace PC} {0.51 0 0.09 0}
\AddSpotColor{PANTONE} {PANTONE306PC} {PANTONE\SpotSpace 306\SpotSpace PC} {0.75 0 0.07 0}
\AddSpotColor{PANTONE} {PANTONE307PC} {PANTONE\SpotSpace 307\SpotSpace PC} {1 0.16 0 0.27}
\AddSpotColor{PANTONE} {PANTONE308PC} {PANTONE\SpotSpace 308\SpotSpace PC} {1 0.05 0 0.47}
\AddSpotColor{PANTONE} {PANTONE309PC} {PANTONE\SpotSpace 309\SpotSpace PC} {1 0 0.09 0.72}
\AddSpotColor{PANTONE} {PANTONE310PC} {PANTONE\SpotSpace 310\SpotSpace PC} {0.43 0 0.1 0}
\AddSpotColor{PANTONE} {PANTONE311PC} {PANTONE\SpotSpace 311\SpotSpace PC} {0.63 0 0.12 0}
\AddSpotColor{PANTONE} {PANTONE312PC} {PANTONE\SpotSpace 312\SpotSpace PC} {0.96 0 0.11 0}
\AddSpotColor{PANTONE} {PANTONE313PC} {PANTONE\SpotSpace 313\SpotSpace PC} {1 0 0.08 0.13}
\AddSpotColor{PANTONE} {PANTONE314PC} {PANTONE\SpotSpace 314\SpotSpace PC} {1 0 0.09 0.3}
\AddSpotColor{PANTONE} {PANTONE315PC} {PANTONE\SpotSpace 315\SpotSpace PC} {1 0 0.12 0.43}
\AddSpotColor{PANTONE} {PANTONE316PC} {PANTONE\SpotSpace 316\SpotSpace PC} {1 0 0.27 0.68}
\AddSpotColor{PANTONE} {PANTONE317PC} {PANTONE\SpotSpace 317\SpotSpace PC} {0.18 0 0.08 0}
\AddSpotColor{PANTONE} {PANTONE318PC} {PANTONE\SpotSpace 318\SpotSpace PC} {0.38 0 0.15 0}
\AddSpotColor{PANTONE} {PANTONE319PC} {PANTONE\SpotSpace 319\SpotSpace PC} {0.52 0 0.19 0}
\AddSpotColor{PANTONE} {PANTONE320PC} {PANTONE\SpotSpace 320\SpotSpace PC} {1 0 0.31 0.07}
\AddSpotColor{PANTONE} {PANTONE321PC} {PANTONE\SpotSpace 321\SpotSpace PC} {1 0 0.31 0.23}
\AddSpotColor{PANTONE} {PANTONE322PC} {PANTONE\SpotSpace 322\SpotSpace PC} {1 0 0.33 0.35}
\AddSpotColor{PANTONE} {PANTONE323PC} {PANTONE\SpotSpace 323\SpotSpace PC} {1 0 0.38 0.47}
\AddSpotColor{PANTONE} {PANTONE324PC} {PANTONE\SpotSpace 324\SpotSpace PC} {0.28 0 0.12 0}
\AddSpotColor{PANTONE} {PANTONE325PC} {PANTONE\SpotSpace 325\SpotSpace PC} {0.56 0 0.26 0}
\AddSpotColor{PANTONE} {PANTONE326PC} {PANTONE\SpotSpace 326\SpotSpace PC} {0.87 0 0.38 0}
\AddSpotColor{PANTONE} {PANTONE327PC} {PANTONE\SpotSpace 327\SpotSpace PC} {1 0 0.44 0.17}
\AddSpotColor{PANTONE} {PANTONE328PC} {PANTONE\SpotSpace 328\SpotSpace PC} {1 0 0.45 0.32}
\AddSpotColor{PANTONE} {PANTONE329PC} {PANTONE\SpotSpace 329\SpotSpace PC} {1 0 0.46 0.46}
\AddSpotColor{PANTONE} {PANTONE330PC} {PANTONE\SpotSpace 330\SpotSpace PC} {1 0 0.48 0.6}
\AddSpotColor{PANTONE} {PANTONE331PC} {PANTONE\SpotSpace 331\SpotSpace PC} {0.24 0 0.16 0}
\AddSpotColor{PANTONE} {PANTONE332PC} {PANTONE\SpotSpace 332\SpotSpace PC} {0.3 0 0.2 0}
\AddSpotColor{PANTONE} {PANTONE333PC} {PANTONE\SpotSpace 333\SpotSpace PC} {0.43 0 0.27 0}
\AddSpotColor{PANTONE} {PANTONE334PC} {PANTONE\SpotSpace 334\SpotSpace PC} {1 0 0.6 0.03}
\AddSpotColor{PANTONE} {PANTONE335PC} {PANTONE\SpotSpace 335\SpotSpace PC} {1 0 0.65 0.3}
\AddSpotColor{PANTONE} {PANTONE336PC} {PANTONE\SpotSpace 336\SpotSpace PC} {1 0 0.67 0.47}
\AddSpotColor{PANTONE} {PANTONE337PC} {PANTONE\SpotSpace 337\SpotSpace PC} {0.31 0 0.2 0}
\AddSpotColor{PANTONE} {PANTONE338PC} {PANTONE\SpotSpace 338\SpotSpace PC} {0.47 0 0.32 0}
\AddSpotColor{PANTONE} {PANTONE339PC} {PANTONE\SpotSpace 339\SpotSpace PC} {0.84 0 0.56 0}
\AddSpotColor{PANTONE} {PANTONE340PC} {PANTONE\SpotSpace 340\SpotSpace PC} {1 0 0.66 0.09}
\AddSpotColor{PANTONE} {PANTONE341PC} {PANTONE\SpotSpace 341\SpotSpace PC} {1 0 0.67 0.29}
\AddSpotColor{PANTONE} {PANTONE342PC} {PANTONE\SpotSpace 342\SpotSpace PC} {1 0 0.71 0.43}
\AddSpotColor{PANTONE} {PANTONE343PC} {PANTONE\SpotSpace 343\SpotSpace PC} {0.98 0 0.72 0.61}
\AddSpotColor{PANTONE} {PANTONE344PC} {PANTONE\SpotSpace 344\SpotSpace PC} {0.27 0 0.23 0}
\AddSpotColor{PANTONE} {PANTONE345PC} {PANTONE\SpotSpace 345\SpotSpace PC} {0.38 0 0.32 0}
\AddSpotColor{PANTONE} {PANTONE346PC} {PANTONE\SpotSpace 346\SpotSpace PC} {0.55 0 0.47 0}
\AddSpotColor{PANTONE} {PANTONE347PC} {PANTONE\SpotSpace 347\SpotSpace PC} {1 0 0.86 0.03}
\AddSpotColor{PANTONE} {PANTONE348PC} {PANTONE\SpotSpace 348\SpotSpace PC} {1 0 0.85 0.24}
\AddSpotColor{PANTONE} {PANTONE349PC} {PANTONE\SpotSpace 349\SpotSpace PC} {1 0 0.91 0.42}
\AddSpotColor{PANTONE} {PANTONE350PC} {PANTONE\SpotSpace 350\SpotSpace PC} {0.79 0 1 0.75}
\AddSpotColor{PANTONE} {PANTONE351PC} {PANTONE\SpotSpace 351\SpotSpace PC} {0.17 0 0.16 0}
\AddSpotColor{PANTONE} {PANTONE352PC} {PANTONE\SpotSpace 352\SpotSpace PC} {0.27 0 0.25 0}
\AddSpotColor{PANTONE} {PANTONE353PC} {PANTONE\SpotSpace 353\SpotSpace PC} {0.38 0 0.36 0}
\AddSpotColor{PANTONE} {PANTONE354PC} {PANTONE\SpotSpace 354\SpotSpace PC} {0.8 0 0.9 0}
\AddSpotColor{PANTONE} {PANTONE355PC} {PANTONE\SpotSpace 355\SpotSpace PC} {0.94 0 1 0}
\AddSpotColor{PANTONE} {PANTONE356PC} {PANTONE\SpotSpace 356\SpotSpace PC} {0.95 0 1 0.27}
\AddSpotColor{PANTONE} {PANTONE357PC} {PANTONE\SpotSpace 357\SpotSpace PC} {0.8 0 1 0.56}
\AddSpotColor{PANTONE} {PANTONE358PC} {PANTONE\SpotSpace 358\SpotSpace PC} {0.27 0 0.38 0}
\AddSpotColor{PANTONE} {PANTONE359PC} {PANTONE\SpotSpace 359\SpotSpace PC} {0.36 0 0.49 0}
\AddSpotColor{PANTONE} {PANTONE360PC} {PANTONE\SpotSpace 360\SpotSpace PC} {0.58 0 0.8 0}
\AddSpotColor{PANTONE} {PANTONE361PC} {PANTONE\SpotSpace 361\SpotSpace PC} {0.69 0 1 0}
\AddSpotColor{PANTONE} {PANTONE362PC} {PANTONE\SpotSpace 362\SpotSpace PC} {0.7 0 1 0.09}
\AddSpotColor{PANTONE} {PANTONE363PC} {PANTONE\SpotSpace 363\SpotSpace PC} {0.68 0 1 0.24}
\AddSpotColor{PANTONE} {PANTONE364PC} {PANTONE\SpotSpace 364\SpotSpace PC} {0.65 0 1 0.42}
\AddSpotColor{PANTONE} {PANTONE365PC} {PANTONE\SpotSpace 365\SpotSpace PC} {0.12 0 0.29 0}
\AddSpotColor{PANTONE} {PANTONE366PC} {PANTONE\SpotSpace 366\SpotSpace PC} {0.2 0 0.44 0}
\AddSpotColor{PANTONE} {PANTONE367PC} {PANTONE\SpotSpace 367\SpotSpace PC} {0.32 0 0.59 0}
\AddSpotColor{PANTONE} {PANTONE368PC} {PANTONE\SpotSpace 368\SpotSpace PC} {0.57 0 1 0}
\AddSpotColor{PANTONE} {PANTONE369PC} {PANTONE\SpotSpace 369\SpotSpace PC} {0.59 0 1 0.07}
\AddSpotColor{PANTONE} {PANTONE370PC} {PANTONE\SpotSpace 370\SpotSpace PC} {0.56 0 1 0.27}
\AddSpotColor{PANTONE} {PANTONE371PC} {PANTONE\SpotSpace 371\SpotSpace PC} {0.43 0 1 0.56}
\AddSpotColor{PANTONE} {PANTONE372PC} {PANTONE\SpotSpace 372\SpotSpace PC} {0.1 0 0.33 0}
\AddSpotColor{PANTONE} {PANTONE373PC} {PANTONE\SpotSpace 373\SpotSpace PC} {0.16 0 0.46 0}
\AddSpotColor{PANTONE} {PANTONE374PC} {PANTONE\SpotSpace 374\SpotSpace PC} {0.24 0 0.57 0}
\AddSpotColor{PANTONE} {PANTONE375PC} {PANTONE\SpotSpace 375\SpotSpace PC} {0.41 0 0.78 0}
\AddSpotColor{PANTONE} {PANTONE376PC} {PANTONE\SpotSpace 376\SpotSpace PC} {0.5 0 1 0}
\AddSpotColor{PANTONE} {PANTONE377PC} {PANTONE\SpotSpace 377\SpotSpace PC} {0.45 0 1 0.24}
\AddSpotColor{PANTONE} {PANTONE378PC} {PANTONE\SpotSpace 378\SpotSpace PC} {0.34 0 1 0.6}
\AddSpotColor{PANTONE} {PANTONE379PC} {PANTONE\SpotSpace 379\SpotSpace PC} {0.09 0 0.58 0}
\AddSpotColor{PANTONE} {PANTONE380PC} {PANTONE\SpotSpace 380\SpotSpace PC} {0.13 0 0.72 0}
\AddSpotColor{PANTONE} {PANTONE381PC} {PANTONE\SpotSpace 381\SpotSpace PC} {0.2 0 0.91 0}
\AddSpotColor{PANTONE} {PANTONE382PC} {PANTONE\SpotSpace 382\SpotSpace PC} {0.29 0 1 0}
\AddSpotColor{PANTONE} {PANTONE383PC} {PANTONE\SpotSpace 383\SpotSpace PC} {0.2 0 1 0.19}
\AddSpotColor{PANTONE} {PANTONE384PC} {PANTONE\SpotSpace 384\SpotSpace PC} {0.18 0 1 0.31}
\AddSpotColor{PANTONE} {PANTONE385PC} {PANTONE\SpotSpace 385\SpotSpace PC} {0.03 0 1 0.58}
\AddSpotColor{PANTONE} {PANTONE386PC} {PANTONE\SpotSpace 386\SpotSpace PC} {0.06 0 0.56 0}
\AddSpotColor{PANTONE} {PANTONE387PC} {PANTONE\SpotSpace 387\SpotSpace PC} {0.1 0 0.74 0}
\AddSpotColor{PANTONE} {PANTONE388PC} {PANTONE\SpotSpace 388\SpotSpace PC} {0.14 0 0.79 0}
\AddSpotColor{PANTONE} {PANTONE389PC} {PANTONE\SpotSpace 389\SpotSpace PC} {0.2 0 0.85 0}
\AddSpotColor{PANTONE} {PANTONE390PC} {PANTONE\SpotSpace 390\SpotSpace PC} {0.22 0 1 0.08}
\AddSpotColor{PANTONE} {PANTONE391PC} {PANTONE\SpotSpace 391\SpotSpace PC} {0.13 0 1 0.33}
\AddSpotColor{PANTONE} {PANTONE392PC} {PANTONE\SpotSpace 392\SpotSpace PC} {0.07 0 1 0.49}
\AddSpotColor{PANTONE} {PANTONE393PC} {PANTONE\SpotSpace 393\SpotSpace PC} {0.03 0 0.55 0}
\AddSpotColor{PANTONE} {PANTONE394PC} {PANTONE\SpotSpace 394\SpotSpace PC} {0.06 0 0.76 0}
\AddSpotColor{PANTONE} {PANTONE395PC} {PANTONE\SpotSpace 395\SpotSpace PC} {0.08 0 0.85 0}
\AddSpotColor{PANTONE} {PANTONE396PC} {PANTONE\SpotSpace 396\SpotSpace PC} {0.11 0 0.94 0}
\AddSpotColor{PANTONE} {PANTONE397PC} {PANTONE\SpotSpace 397\SpotSpace PC} {0.1 0 1 0.11}
\AddSpotColor{PANTONE} {PANTONE398PC} {PANTONE\SpotSpace 398\SpotSpace PC} {0.07 0 1 0.28}
\AddSpotColor{PANTONE} {PANTONE399PC} {PANTONE\SpotSpace 399\SpotSpace PC} {0 0 1 0.43}
\AddSpotColor{PANTONE} {PANTONE400PC} {PANTONE\SpotSpace 400\SpotSpace PC} {0 0.03 0.06 0.16}
\AddSpotColor{PANTONE} {PANTONE401PC} {PANTONE\SpotSpace 401\SpotSpace PC} {0 0.05 0.11 0.23}
\AddSpotColor{PANTONE} {PANTONE402PC} {PANTONE\SpotSpace 402\SpotSpace PC} {0 0.06 0.14 0.31}
\AddSpotColor{PANTONE} {PANTONE403PC} {PANTONE\SpotSpace 403\SpotSpace PC} {0 0.07 0.17 0.43}
\AddSpotColor{PANTONE} {PANTONE404PC} {PANTONE\SpotSpace 404\SpotSpace PC} {0 0.08 0.22 0.56}
\AddSpotColor{PANTONE} {PANTONE405PC} {PANTONE\SpotSpace 405\SpotSpace PC} {0 0.1 0.33 0.72}
\AddSpotColor{PANTONE} {PANTONE406PC} {PANTONE\SpotSpace 406\SpotSpace PC} {0 0.05 0.06 0.16}
\AddSpotColor{PANTONE} {PANTONE407PC} {PANTONE\SpotSpace 407\SpotSpace PC} {0 0.08 0.09 0.26}
\AddSpotColor{PANTONE} {PANTONE408PC} {PANTONE\SpotSpace 408\SpotSpace PC} {0 0.1 0.11 0.34}
\AddSpotColor{PANTONE} {PANTONE409PC} {PANTONE\SpotSpace 409\SpotSpace PC} {0 0.13 0.15 0.45}
\AddSpotColor{PANTONE} {PANTONE410PC} {PANTONE\SpotSpace 410\SpotSpace PC} {0 0.18 0.21 0.56}
\AddSpotColor{PANTONE} {PANTONE411PC} {PANTONE\SpotSpace 411\SpotSpace PC} {0 0.27 0.36 0.72}
\AddSpotColor{PANTONE} {PANTONE412PC} {PANTONE\SpotSpace 412\SpotSpace PC} {0 0.3 0.66 0.98}
\AddSpotColor{PANTONE} {PANTONE413PC} {PANTONE\SpotSpace 413\SpotSpace PC} {0 0 0.09 0.2}
\AddSpotColor{PANTONE} {PANTONE414PC} {PANTONE\SpotSpace 414\SpotSpace PC} {0 0 0.1 0.3}
\AddSpotColor{PANTONE} {PANTONE415PC} {PANTONE\SpotSpace 415\SpotSpace PC} {0 0 0.12 0.41}
\AddSpotColor{PANTONE} {PANTONE416PC} {PANTONE\SpotSpace 416\SpotSpace PC} {0 0 0.16 0.5}
\AddSpotColor{PANTONE} {PANTONE417PC} {PANTONE\SpotSpace 417\SpotSpace PC} {0.01 0 0.25 0.65}
\AddSpotColor{PANTONE} {PANTONE418PC} {PANTONE\SpotSpace 418\SpotSpace PC} {0.03 0 0.31 0.75}
\AddSpotColor{PANTONE} {PANTONE419PC} {PANTONE\SpotSpace 419\SpotSpace PC} {0.29 0 0.36 1}
\AddSpotColor{PANTONE} {PANTONE420PC} {PANTONE\SpotSpace 420\SpotSpace PC} {0 0 0 0.15}
\AddSpotColor{PANTONE} {PANTONE421PC} {PANTONE\SpotSpace 421\SpotSpace PC} {0 0 0 0.26}
\AddSpotColor{PANTONE} {PANTONE422PC} {PANTONE\SpotSpace 422\SpotSpace PC} {0 0 0 0.33}
\AddSpotColor{PANTONE} {PANTONE423PC} {PANTONE\SpotSpace 423\SpotSpace PC} {0 0 0 0.44}
\AddSpotColor{PANTONE} {PANTONE424PC} {PANTONE\SpotSpace 424\SpotSpace PC} {0 0 0 0.61}
\AddSpotColor{PANTONE} {PANTONE425PC} {PANTONE\SpotSpace 425\SpotSpace PC} {0 0 0 0.77}
\AddSpotColor{PANTONE} {PANTONE426PC} {PANTONE\SpotSpace 426\SpotSpace PC} {0 0 0 0.99}
\AddSpotColor{PANTONE} {PANTONE427PC} {PANTONE\SpotSpace 427\SpotSpace PC} {0 0 0 0.11}
\AddSpotColor{PANTONE} {PANTONE428PC} {PANTONE\SpotSpace 428\SpotSpace PC} {0.02 0 0 0.18}
\AddSpotColor{PANTONE} {PANTONE429PC} {PANTONE\SpotSpace 429\SpotSpace PC} {0.03 0 0 0.32}
\AddSpotColor{PANTONE} {PANTONE430PC} {PANTONE\SpotSpace 430\SpotSpace PC} {0.05 0 0 0.45}
\AddSpotColor{PANTONE} {PANTONE431PC} {PANTONE\SpotSpace 431\SpotSpace PC} {0.11 0.01 0 0.64}
\AddSpotColor{PANTONE} {PANTONE432PC} {PANTONE\SpotSpace 432\SpotSpace PC} {0.23 0.02 0 0.77}
\AddSpotColor{PANTONE} {PANTONE433PC} {PANTONE\SpotSpace 433\SpotSpace PC} {0.33 0.03 0 0.95}
\AddSpotColor{PANTONE} {PANTONE434PC} {PANTONE\SpotSpace 434\SpotSpace PC} {0.07 0.09 0.1 0}
\AddSpotColor{PANTONE} {PANTONE435PC} {PANTONE\SpotSpace 435\SpotSpace PC} {0.13 0.15 0.15 0}
\AddSpotColor{PANTONE} {PANTONE436PC} {PANTONE\SpotSpace 436\SpotSpace PC} {0.24 0.25 0.26 0}
\AddSpotColor{PANTONE} {PANTONE437PC} {PANTONE\SpotSpace 437\SpotSpace PC} {0.46 0.45 0.49 0}
\AddSpotColor{PANTONE} {PANTONE438PC} {PANTONE\SpotSpace 438\SpotSpace PC} {0.75 0.68 1 0.1}
\AddSpotColor{PANTONE} {PANTONE439PC} {PANTONE\SpotSpace 439\SpotSpace PC} {0.8 0.73 1 0.2}
\AddSpotColor{PANTONE} {PANTONE440PC} {PANTONE\SpotSpace 440\SpotSpace PC} {0.82 0.76 1 0.3}
\AddSpotColor{PANTONE} {PANTONE441PC} {PANTONE\SpotSpace 441\SpotSpace PC} {0.06 0 0.07 0.09}
\AddSpotColor{PANTONE} {PANTONE442PC} {PANTONE\SpotSpace 442\SpotSpace PC} {0.08 0 0.09 0.19}
\AddSpotColor{PANTONE} {PANTONE443PC} {PANTONE\SpotSpace 443\SpotSpace PC} {0.12 0 0.12 0.3}
\AddSpotColor{PANTONE} {PANTONE444PC} {PANTONE\SpotSpace 444\SpotSpace PC} {0.15 0 0.15 0.42}
\AddSpotColor{PANTONE} {PANTONE445PC} {PANTONE\SpotSpace 445\SpotSpace PC} {0.2 0 0.2 0.65}
\AddSpotColor{PANTONE} {PANTONE446PC} {PANTONE\SpotSpace 446\SpotSpace PC} {0.21 0 0.23 0.75}
\AddSpotColor{PANTONE} {PANTONE447PC} {PANTONE\SpotSpace 447\SpotSpace PC} {0.16 0 0.31 0.82}
\AddSpotColor{PANTONE} {PANTONE448PC} {PANTONE\SpotSpace 448\SpotSpace PC} {0.65 0.58 1 0.35}
\AddSpotColor{PANTONE} {PANTONE449PC} {PANTONE\SpotSpace 449\SpotSpace PC} {0.65 0.55 1 0.28}
\AddSpotColor{PANTONE} {PANTONE450PC} {PANTONE\SpotSpace 450\SpotSpace PC} {0.6 0.5 1 0.22}
\AddSpotColor{PANTONE} {PANTONE451PC} {PANTONE\SpotSpace 451\SpotSpace PC} {0.33 0.28 0.58 0}
\AddSpotColor{PANTONE} {PANTONE452PC} {PANTONE\SpotSpace 452\SpotSpace PC} {0.24 0.18 0.42 0}
\AddSpotColor{PANTONE} {PANTONE453PC} {PANTONE\SpotSpace 453\SpotSpace PC} {0.14 0.1 0.27 0}
\AddSpotColor{PANTONE} {PANTONE454PC} {PANTONE\SpotSpace 454\SpotSpace PC} {0.09 0.06 0.17 0}
\AddSpotColor{PANTONE} {PANTONE455PC} {PANTONE\SpotSpace 455\SpotSpace PC} {0 0.17 1 0.65}
\AddSpotColor{PANTONE} {PANTONE456PC} {PANTONE\SpotSpace 456\SpotSpace PC} {0 0.15 1 0.43}
\AddSpotColor{PANTONE} {PANTONE457PC} {PANTONE\SpotSpace 457\SpotSpace PC} {0 0.15 1 0.28}
\AddSpotColor{PANTONE} {PANTONE458PC} {PANTONE\SpotSpace 458\SpotSpace PC} {0.1 0.1 0.73 0}
\AddSpotColor{PANTONE} {PANTONE459PC} {PANTONE\SpotSpace 459\SpotSpace PC} {0.06 0.07 0.55 0}
\AddSpotColor{PANTONE} {PANTONE460PC} {PANTONE\SpotSpace 460\SpotSpace PC} {0.04 0.05 0.44 0}
\AddSpotColor{PANTONE} {PANTONE461PC} {PANTONE\SpotSpace 461\SpotSpace PC} {0.03 0.03 0.35 0}
\AddSpotColor{PANTONE} {PANTONE462PC} {PANTONE\SpotSpace 462\SpotSpace PC} {0.5 0.58 1 0.45}
\AddSpotColor{PANTONE} {PANTONE463PC} {PANTONE\SpotSpace 463\SpotSpace PC} {0.3 0.56 1 0.37}
\AddSpotColor{PANTONE} {PANTONE464PC} {PANTONE\SpotSpace 464\SpotSpace PC} {0.1 0.49 1 0.35}
\AddSpotColor{PANTONE} {PANTONE465PC} {PANTONE\SpotSpace 465\SpotSpace PC} {0.2 0.32 0.58 0}
\AddSpotColor{PANTONE} {PANTONE466PC} {PANTONE\SpotSpace 466\SpotSpace PC} {0.12 0.22 0.43 0}
\AddSpotColor{PANTONE} {PANTONE467PC} {PANTONE\SpotSpace 467\SpotSpace PC} {0.09 0.15 0.34 0}
\AddSpotColor{PANTONE} {PANTONE468PC} {PANTONE\SpotSpace 468\SpotSpace PC} {0.06 0.09 0.23 0}
\AddSpotColor{PANTONE} {PANTONE469PC} {PANTONE\SpotSpace 469\SpotSpace PC} {0 0.52 1 0.62}
\AddSpotColor{PANTONE} {PANTONE470PC} {PANTONE\SpotSpace 470\SpotSpace PC} {0 0.58 1 0.33}
\AddSpotColor{PANTONE} {PANTONE471PC} {PANTONE\SpotSpace 471\SpotSpace PC} {0 0.59 1 0.18}
\AddSpotColor{PANTONE} {PANTONE472PC} {PANTONE\SpotSpace 472\SpotSpace PC} {0 0.34 0.52 0}
\AddSpotColor{PANTONE} {PANTONE473PC} {PANTONE\SpotSpace 473\SpotSpace PC} {0 0.23 0.36 0}
\AddSpotColor{PANTONE} {PANTONE474PC} {PANTONE\SpotSpace 474\SpotSpace PC} {0 0.15 0.26 0}
\AddSpotColor{PANTONE} {PANTONE475PC} {PANTONE\SpotSpace 475\SpotSpace PC} {0 0.11 0.2 0}
\AddSpotColor{PANTONE} {PANTONE476PC} {PANTONE\SpotSpace 476\SpotSpace PC} {0.57 0.8 1 0.45}
\AddSpotColor{PANTONE} {PANTONE477PC} {PANTONE\SpotSpace 477\SpotSpace PC} {0.5 0.85 1 0.35}
\AddSpotColor{PANTONE} {PANTONE478PC} {PANTONE\SpotSpace 478\SpotSpace PC} {0.4 0.86 1 0.3}
\AddSpotColor{PANTONE} {PANTONE479PC} {PANTONE\SpotSpace 479\SpotSpace PC} {0.3 0.48 0.57 0}
\AddSpotColor{PANTONE} {PANTONE480PC} {PANTONE\SpotSpace 480\SpotSpace PC} {0.15 0.29 0.33 0}
\AddSpotColor{PANTONE} {PANTONE481PC} {PANTONE\SpotSpace 481\SpotSpace PC} {0.09 0.19 0.23 0}
\AddSpotColor{PANTONE} {PANTONE482PC} {PANTONE\SpotSpace 482\SpotSpace PC} {0.05 0.11 0.15 0}
\AddSpotColor{PANTONE} {PANTONE483PC} {PANTONE\SpotSpace 483\SpotSpace PC} {0 0.91 1 0.6}
\AddSpotColor{PANTONE} {PANTONE484PC} {PANTONE\SpotSpace 484\SpotSpace PC} {0 0.95 1 0.29}
\AddSpotColor{PANTONE} {PANTONE485PC} {PANTONE\SpotSpace 485\SpotSpace PC} {0 0.95 1 0}
\AddSpotColor{PANTONE} {PANTONE486PC} {PANTONE\SpotSpace 486\SpotSpace PC} {0 0.47 0.41 0}
\AddSpotColor{PANTONE} {PANTONE487PC} {PANTONE\SpotSpace 487\SpotSpace PC} {0 0.35 0.28 0}
\AddSpotColor{PANTONE} {PANTONE488PC} {PANTONE\SpotSpace 488\SpotSpace PC} {0 0.26 0.19 0}
\AddSpotColor{PANTONE} {PANTONE489PC} {PANTONE\SpotSpace 489\SpotSpace PC} {0 0.15 0.11 0}
\AddSpotColor{PANTONE} {PANTONE490PC} {PANTONE\SpotSpace 490\SpotSpace PC} {0 0.74 1 0.72}
\AddSpotColor{PANTONE} {PANTONE491PC} {PANTONE\SpotSpace 491\SpotSpace PC} {0 0.79 1 0.52}
\AddSpotColor{PANTONE} {PANTONE492PC} {PANTONE\SpotSpace 492\SpotSpace PC} {0 0.7 0.66 0.3}
\AddSpotColor{PANTONE} {PANTONE493PC} {PANTONE\SpotSpace 493\SpotSpace PC} {0 0.46 0.23 0.05}
\AddSpotColor{PANTONE} {PANTONE494PC} {PANTONE\SpotSpace 494\SpotSpace PC} {0 0.33 0.13 0}
\AddSpotColor{PANTONE} {PANTONE495PC} {PANTONE\SpotSpace 495\SpotSpace PC} {0 0.24 0.11 0}
\AddSpotColor{PANTONE} {PANTONE496PC} {PANTONE\SpotSpace 496\SpotSpace PC} {0 0.16 0.09 0}
\AddSpotColor{PANTONE} {PANTONE497PC} {PANTONE\SpotSpace 497\SpotSpace PC} {0 0.7 1 0.78}
\AddSpotColor{PANTONE} {PANTONE498PC} {PANTONE\SpotSpace 498\SpotSpace PC} {0 0.64 1 0.6}
\AddSpotColor{PANTONE} {PANTONE499PC} {PANTONE\SpotSpace 499\SpotSpace PC} {0 0.58 1 0.49}
\AddSpotColor{PANTONE} {PANTONE500PC} {PANTONE\SpotSpace 500\SpotSpace PC} {0 0.38 0.21 0.11}
\AddSpotColor{PANTONE} {PANTONE501PC} {PANTONE\SpotSpace 501\SpotSpace PC} {0 0.27 0.13 0.03}
\AddSpotColor{PANTONE} {PANTONE502PC} {PANTONE\SpotSpace 502\SpotSpace PC} {0 0.18 0.1 0.01}
\AddSpotColor{PANTONE} {PANTONE503PC} {PANTONE\SpotSpace 503\SpotSpace PC} {0 0.11 0.08 0}
\AddSpotColor{PANTONE} {PANTONE504PC} {PANTONE\SpotSpace 504\SpotSpace PC} {0.65 1 1 0.35}
\AddSpotColor{PANTONE} {PANTONE505PC} {PANTONE\SpotSpace 505\SpotSpace PC} {0.5 1 1 0.25}
\AddSpotColor{PANTONE} {PANTONE506PC} {PANTONE\SpotSpace 506\SpotSpace PC} {0.45 1 1 0.15}
\AddSpotColor{PANTONE} {PANTONE507PC} {PANTONE\SpotSpace 507\SpotSpace PC} {0.11 0.45 0.22 0}
\AddSpotColor{PANTONE} {PANTONE508PC} {PANTONE\SpotSpace 508\SpotSpace PC} {0.04 0.34 0.11 0}
\AddSpotColor{PANTONE} {PANTONE509PC} {PANTONE\SpotSpace 509\SpotSpace PC} {0 0.24 0.07 0}
\AddSpotColor{PANTONE} {PANTONE510PC} {PANTONE\SpotSpace 510\SpotSpace PC} {0 0.17 0.06 0}
\AddSpotColor{PANTONE} {PANTONE511PC} {PANTONE\SpotSpace 511\SpotSpace PC} {0.6 1 0.45 0.3}
\AddSpotColor{PANTONE} {PANTONE512PC} {PANTONE\SpotSpace 512\SpotSpace PC} {0.5 1 0.15 0.1}
\AddSpotColor{PANTONE} {PANTONE513PC} {PANTONE\SpotSpace 513\SpotSpace PC} {0.44 0.83 0 0}
\AddSpotColor{PANTONE} {PANTONE514PC} {PANTONE\SpotSpace 514\SpotSpace PC} {0.15 0.5 0 0}
\AddSpotColor{PANTONE} {PANTONE515PC} {PANTONE\SpotSpace 515\SpotSpace PC} {0.07 0.38 0 0}
\AddSpotColor{PANTONE} {PANTONE516PC} {PANTONE\SpotSpace 516\SpotSpace PC} {0.03 0.27 0 0}
\AddSpotColor{PANTONE} {PANTONE517PC} {PANTONE\SpotSpace 517\SpotSpace PC} {0 0.18 0 0}
\AddSpotColor{PANTONE} {PANTONE518PC} {PANTONE\SpotSpace 518\SpotSpace PC} {0.7 1 0.55 0.25}
\AddSpotColor{PANTONE} {PANTONE519PC} {PANTONE\SpotSpace 519\SpotSpace PC} {0.67 1 0.3 0.1}
\AddSpotColor{PANTONE} {PANTONE520PC} {PANTONE\SpotSpace 520\SpotSpace PC} {0.64 1 0.12 0}
\AddSpotColor{PANTONE} {PANTONE521PC} {PANTONE\SpotSpace 521\SpotSpace PC} {0.27 0.47 0 0}
\AddSpotColor{PANTONE} {PANTONE522PC} {PANTONE\SpotSpace 522\SpotSpace PC} {0.17 0.37 0 0}
\AddSpotColor{PANTONE} {PANTONE523PC} {PANTONE\SpotSpace 523\SpotSpace PC} {0.1 0.26 0 0}
\AddSpotColor{PANTONE} {PANTONE524PC} {PANTONE\SpotSpace 524\SpotSpace PC} {0.06 0.15 0 0}
\AddSpotColor{PANTONE} {PANTONE525PC} {PANTONE\SpotSpace 525\SpotSpace PC} {0.84 1 0.45 0.05}
\AddSpotColor{PANTONE} {PANTONE526PC} {PANTONE\SpotSpace 526\SpotSpace PC} {0.76 1 0.07 0}
\AddSpotColor{PANTONE} {PANTONE527PC} {PANTONE\SpotSpace 527\SpotSpace PC} {0.73 1 0 0}
\AddSpotColor{PANTONE} {PANTONE528PC} {PANTONE\SpotSpace 528\SpotSpace PC} {0.41 0.55 0 0}
\AddSpotColor{PANTONE} {PANTONE529PC} {PANTONE\SpotSpace 529\SpotSpace PC} {0.26 0.4 0 0}
\AddSpotColor{PANTONE} {PANTONE530PC} {PANTONE\SpotSpace 530\SpotSpace PC} {0.18 0.31 0 0}
\AddSpotColor{PANTONE} {PANTONE531PC} {PANTONE\SpotSpace 531\SpotSpace PC} {0.1 0.2 0 0}
\AddSpotColor{PANTONE} {PANTONE532PC} {PANTONE\SpotSpace 532\SpotSpace PC} {1 0.8 0.7 0.25}
\AddSpotColor{PANTONE} {PANTONE533PC} {PANTONE\SpotSpace 533\SpotSpace PC} {1 0.83 0.46 0.13}
\AddSpotColor{PANTONE} {PANTONE534PC} {PANTONE\SpotSpace 534\SpotSpace PC} {1 0.8 0.3 0.05}
\AddSpotColor{PANTONE} {PANTONE535PC} {PANTONE\SpotSpace 535\SpotSpace PC} {0.42 0.27 0.07 0}
\AddSpotColor{PANTONE} {PANTONE536PC} {PANTONE\SpotSpace 536\SpotSpace PC} {0.31 0.2 0.05 0}
\AddSpotColor{PANTONE} {PANTONE537PC} {PANTONE\SpotSpace 537\SpotSpace PC} {0.22 0.12 0.03 0}
\AddSpotColor{PANTONE} {PANTONE538PC} {PANTONE\SpotSpace 538\SpotSpace PC} {0.12 0.07 0.02 0}
\AddSpotColor{PANTONE} {PANTONE539PC} {PANTONE\SpotSpace 539\SpotSpace PC} {1 0.49 0 0.7}
\AddSpotColor{PANTONE} {PANTONE540PC} {PANTONE\SpotSpace 540\SpotSpace PC} {1 0.55 0 0.55}
\AddSpotColor{PANTONE} {PANTONE541PC} {PANTONE\SpotSpace 541\SpotSpace PC} {1 0.57 0 0.38}
\AddSpotColor{PANTONE} {PANTONE542PC} {PANTONE\SpotSpace 542\SpotSpace PC} {0.62 0.22 0 0.03}
\AddSpotColor{PANTONE} {PANTONE543PC} {PANTONE\SpotSpace 543\SpotSpace PC} {0.41 0.11 0 0}
\AddSpotColor{PANTONE} {PANTONE544PC} {PANTONE\SpotSpace 544\SpotSpace PC} {0.3 0.06 0 0}
\AddSpotColor{PANTONE} {PANTONE545PC} {PANTONE\SpotSpace 545\SpotSpace PC} {0.22 0.03 0 0}
\AddSpotColor{PANTONE} {PANTONE546PC} {PANTONE\SpotSpace 546\SpotSpace PC} {0.95 0.09 0 0.83}
\AddSpotColor{PANTONE} {PANTONE547PC} {PANTONE\SpotSpace 547\SpotSpace PC} {1 0.19 0 0.75}
\AddSpotColor{PANTONE} {PANTONE548PC} {PANTONE\SpotSpace 548\SpotSpace PC} {1 0.24 0 0.64}
\AddSpotColor{PANTONE} {PANTONE549PC} {PANTONE\SpotSpace 549\SpotSpace PC} {0.52 0.06 0 0.25}
\AddSpotColor{PANTONE} {PANTONE550PC} {PANTONE\SpotSpace 550\SpotSpace PC} {0.38 0.04 0 0.19}
\AddSpotColor{PANTONE} {PANTONE551PC} {PANTONE\SpotSpace 551\SpotSpace PC} {0.27 0.03 0 0.13}
\AddSpotColor{PANTONE} {PANTONE552PC} {PANTONE\SpotSpace 552\SpotSpace PC} {0.15 0 0 0.09}
\AddSpotColor{PANTONE} {PANTONE553PC} {PANTONE\SpotSpace 553\SpotSpace PC} {0.59 0 0.53 0.8}
\AddSpotColor{PANTONE} {PANTONE554PC} {PANTONE\SpotSpace 554\SpotSpace PC} {0.78 0 0.63 0.67}
\AddSpotColor{PANTONE} {PANTONE555PC} {PANTONE\SpotSpace 555\SpotSpace PC} {0.75 0 0.6 0.55}
\AddSpotColor{PANTONE} {PANTONE556PC} {PANTONE\SpotSpace 556\SpotSpace PC} {0.42 0 0.33 0.27}
\AddSpotColor{PANTONE} {PANTONE557PC} {PANTONE\SpotSpace 557\SpotSpace PC} {0.3 0 0.2 0.15}
\AddSpotColor{PANTONE} {PANTONE558PC} {PANTONE\SpotSpace 558\SpotSpace PC} {0.19 0 0.14 0.09}
\AddSpotColor{PANTONE} {PANTONE559PC} {PANTONE\SpotSpace 559\SpotSpace PC} {0.14 0 0.1 0.06}
\AddSpotColor{PANTONE} {PANTONE560PC} {PANTONE\SpotSpace 560\SpotSpace PC} {0.8 0 0.63 0.75}
\AddSpotColor{PANTONE} {PANTONE561PC} {PANTONE\SpotSpace 561\SpotSpace PC} {0.85 0 0.54 0.52}
\AddSpotColor{PANTONE} {PANTONE562PC} {PANTONE\SpotSpace 562\SpotSpace PC} {0.85 0 0.5 0.31}
\AddSpotColor{PANTONE} {PANTONE563PC} {PANTONE\SpotSpace 563\SpotSpace PC} {0.52 0 0.32 0.01}
\AddSpotColor{PANTONE} {PANTONE564PC} {PANTONE\SpotSpace 564\SpotSpace PC} {0.37 0 0.2 0}
\AddSpotColor{PANTONE} {PANTONE565PC} {PANTONE\SpotSpace 565\SpotSpace PC} {0.23 0 0.13 0}
\AddSpotColor{PANTONE} {PANTONE566PC} {PANTONE\SpotSpace 566\SpotSpace PC} {0.14 0 0.1 0}
\AddSpotColor{PANTONE} {PANTONE567PC} {PANTONE\SpotSpace 567\SpotSpace PC} {0.82 0 0.64 0.7}
\AddSpotColor{PANTONE} {PANTONE568PC} {PANTONE\SpotSpace 568\SpotSpace PC} {0.88 0 0.57 0.36}
\AddSpotColor{PANTONE} {PANTONE569PC} {PANTONE\SpotSpace 569\SpotSpace PC} {0.98 0 0.57 0.17}
\AddSpotColor{PANTONE} {PANTONE570PC} {PANTONE\SpotSpace 570\SpotSpace PC} {0.48 0 0.29 0}
\AddSpotColor{PANTONE} {PANTONE571PC} {PANTONE\SpotSpace 571\SpotSpace PC} {0.32 0 0.19 0}
\AddSpotColor{PANTONE} {PANTONE572PC} {PANTONE\SpotSpace 572\SpotSpace PC} {0.23 0 0.14 0}
\AddSpotColor{PANTONE} {PANTONE573PC} {PANTONE\SpotSpace 573\SpotSpace PC} {0.14 0 0.09 0}
\AddSpotColor{PANTONE} {PANTONE574PC} {PANTONE\SpotSpace 574\SpotSpace PC} {0.34 0 0.81 0.71}
\AddSpotColor{PANTONE} {PANTONE575PC} {PANTONE\SpotSpace 575\SpotSpace PC} {0.48 0 1 0.53}
\AddSpotColor{PANTONE} {PANTONE576PC} {PANTONE\SpotSpace 576\SpotSpace PC} {0.49 0 1 0.39}
\AddSpotColor{PANTONE} {PANTONE577PC} {PANTONE\SpotSpace 577\SpotSpace PC} {0.24 0 0.46 0.1}
\AddSpotColor{PANTONE} {PANTONE578PC} {PANTONE\SpotSpace 578\SpotSpace PC} {0.2 0 0.4 0.06}
\AddSpotColor{PANTONE} {PANTONE579PC} {PANTONE\SpotSpace 579\SpotSpace PC} {0.17 0 0.34 0.03}
\AddSpotColor{PANTONE} {PANTONE580PC} {PANTONE\SpotSpace 580\SpotSpace PC} {0.12 0 0.26 0.02}
\AddSpotColor{PANTONE} {PANTONE581PC} {PANTONE\SpotSpace 581\SpotSpace PC} {0.02 0 1 0.72}
\AddSpotColor{PANTONE} {PANTONE582PC} {PANTONE\SpotSpace 582\SpotSpace PC} {0.13 0 1 0.46}
\AddSpotColor{PANTONE} {PANTONE583PC} {PANTONE\SpotSpace 583\SpotSpace PC} {0.23 0 1 0.17}
\AddSpotColor{PANTONE} {PANTONE584PC} {PANTONE\SpotSpace 584\SpotSpace PC} {0.12 0 0.79 0.06}
\AddSpotColor{PANTONE} {PANTONE585PC} {PANTONE\SpotSpace 585\SpotSpace PC} {0.11 0 0.66 0.02}
\AddSpotColor{PANTONE} {PANTONE586PC} {PANTONE\SpotSpace 586\SpotSpace PC} {0.09 0 0.53 0}
\AddSpotColor{PANTONE} {PANTONE587PC} {PANTONE\SpotSpace 587\SpotSpace PC} {0.05 0 0.4 0}
\AddSpotColor{PANTONE} {PANTONE600PC} {PANTONE\SpotSpace 600\SpotSpace PC} {0 0 0.29 0}
\AddSpotColor{PANTONE} {PANTONE601PC} {PANTONE\SpotSpace 601\SpotSpace PC} {0 0 0.4 0}
\AddSpotColor{PANTONE} {PANTONE602PC} {PANTONE\SpotSpace 602\SpotSpace PC} {0 0 0.5 0}
\AddSpotColor{PANTONE} {PANTONE603PC} {PANTONE\SpotSpace 603\SpotSpace PC} {0 0 0.69 0.01}
\AddSpotColor{PANTONE} {PANTONE604PC} {PANTONE\SpotSpace 604\SpotSpace PC} {0 0 0.88 0.03}
\AddSpotColor{PANTONE} {PANTONE605PC} {PANTONE\SpotSpace 605\SpotSpace PC} {0 0.02 1 0.07}
\AddSpotColor{PANTONE} {PANTONE606PC} {PANTONE\SpotSpace 606\SpotSpace PC} {0 0.04 1 0.12}
\AddSpotColor{PANTONE} {PANTONE607PC} {PANTONE\SpotSpace 607\SpotSpace PC} {0 0 0.18 0.01}
\AddSpotColor{PANTONE} {PANTONE608PC} {PANTONE\SpotSpace 608\SpotSpace PC} {0 0 0.32 0.02}
\AddSpotColor{PANTONE} {PANTONE609PC} {PANTONE\SpotSpace 609\SpotSpace PC} {0 0 0.46 0.04}
\AddSpotColor{PANTONE} {PANTONE610PC} {PANTONE\SpotSpace 610\SpotSpace PC} {0 0 0.58 0.06}
\AddSpotColor{PANTONE} {PANTONE611PC} {PANTONE\SpotSpace 611\SpotSpace PC} {0 0.01 0.92 0.11}
\AddSpotColor{PANTONE} {PANTONE612PC} {PANTONE\SpotSpace 612\SpotSpace PC} {0 0.02 1 0.2}
\AddSpotColor{PANTONE} {PANTONE613PC} {PANTONE\SpotSpace 613\SpotSpace PC} {0 0.04 1 0.3}
\AddSpotColor{PANTONE} {PANTONE614PC} {PANTONE\SpotSpace 614\SpotSpace PC} {0 0 0.2 0.04}
\AddSpotColor{PANTONE} {PANTONE615PC} {PANTONE\SpotSpace 615\SpotSpace PC} {0 0.01 0.27 0.06}
\AddSpotColor{PANTONE} {PANTONE616PC} {PANTONE\SpotSpace 616\SpotSpace PC} {0 0.02 0.35 0.09}
\AddSpotColor{PANTONE} {PANTONE617PC} {PANTONE\SpotSpace 617\SpotSpace PC} {0 0.02 0.48 0.17}
\AddSpotColor{PANTONE} {PANTONE618PC} {PANTONE\SpotSpace 618\SpotSpace PC} {0 0.03 0.87 0.3}
\AddSpotColor{PANTONE} {PANTONE619PC} {PANTONE\SpotSpace 619\SpotSpace PC} {0 0.04 1 0.43}
\AddSpotColor{PANTONE} {PANTONE620PC} {PANTONE\SpotSpace 620\SpotSpace PC} {0 0.05 1 0.53}
\AddSpotColor{PANTONE} {PANTONE621PC} {PANTONE\SpotSpace 621\SpotSpace PC} {0.13 0 0.1 0.02}
\AddSpotColor{PANTONE} {PANTONE622PC} {PANTONE\SpotSpace 622\SpotSpace PC} {0.24 0 0.19 0.04}
\AddSpotColor{PANTONE} {PANTONE623PC} {PANTONE\SpotSpace 623\SpotSpace PC} {0.32 0 0.24 0.1}
\AddSpotColor{PANTONE} {PANTONE624PC} {PANTONE\SpotSpace 624\SpotSpace PC} {0.44 0 0.35 0.2}
\AddSpotColor{PANTONE} {PANTONE625PC} {PANTONE\SpotSpace 625\SpotSpace PC} {0.56 0 0.44 0.33}
\AddSpotColor{PANTONE} {PANTONE626PC} {PANTONE\SpotSpace 626\SpotSpace PC} {0.76 0 0.64 0.62}
\AddSpotColor{PANTONE} {PANTONE627PC} {PANTONE\SpotSpace 627\SpotSpace PC} {0.9 0 0.75 0.83}
\AddSpotColor{PANTONE} {PANTONE628PC} {PANTONE\SpotSpace 628\SpotSpace PC} {0.19 0 0.06 0}
\AddSpotColor{PANTONE} {PANTONE629PC} {PANTONE\SpotSpace 629\SpotSpace PC} {0.34 0 0.09 0}
\AddSpotColor{PANTONE} {PANTONE630PC} {PANTONE\SpotSpace 630\SpotSpace PC} {0.47 0 0.11 0}
\AddSpotColor{PANTONE} {PANTONE631PC} {PANTONE\SpotSpace 631\SpotSpace PC} {0.67 0 0.12 0.02}
\AddSpotColor{PANTONE} {PANTONE632PC} {PANTONE\SpotSpace 632\SpotSpace PC} {0.92 0 0.15 0.05}
\AddSpotColor{PANTONE} {PANTONE633PC} {PANTONE\SpotSpace 633\SpotSpace PC} {1 0 0.1 0.25}
\AddSpotColor{PANTONE} {PANTONE634PC} {PANTONE\SpotSpace 634\SpotSpace PC} {1 0 0.09 0.4}
\AddSpotColor{PANTONE} {PANTONE635PC} {PANTONE\SpotSpace 635\SpotSpace PC} {0.32 0 0.08 0}
\AddSpotColor{PANTONE} {PANTONE636PC} {PANTONE\SpotSpace 636\SpotSpace PC} {0.45 0 0.09 0}
\AddSpotColor{PANTONE} {PANTONE637PC} {PANTONE\SpotSpace 637\SpotSpace PC} {0.55 0 0.09 0}
\AddSpotColor{PANTONE} {PANTONE638PC} {PANTONE\SpotSpace 638\SpotSpace PC} {0.83 0 0.1 0}
\AddSpotColor{PANTONE} {PANTONE639PC} {PANTONE\SpotSpace 639\SpotSpace PC} {1 0 0.05 0.05}
\AddSpotColor{PANTONE} {PANTONE640PC} {PANTONE\SpotSpace 640\SpotSpace PC} {1 0 0 0.22}
\AddSpotColor{PANTONE} {PANTONE641PC} {PANTONE\SpotSpace 641\SpotSpace PC} {1 0.04 0 0.3}
\AddSpotColor{PANTONE} {PANTONE642PC} {PANTONE\SpotSpace 642\SpotSpace PC} {0.16 0.04 0 0.02}
\AddSpotColor{PANTONE} {PANTONE643PC} {PANTONE\SpotSpace 643\SpotSpace PC} {0.25 0.07 0 0.04}
\AddSpotColor{PANTONE} {PANTONE644PC} {PANTONE\SpotSpace 644\SpotSpace PC} {0.42 0.15 0 0.06}
\AddSpotColor{PANTONE} {PANTONE645PC} {PANTONE\SpotSpace 645\SpotSpace PC} {0.55 0.24 0 0.09}
\AddSpotColor{PANTONE} {PANTONE646PC} {PANTONE\SpotSpace 646\SpotSpace PC} {0.65 0.3 0 0.11}
\AddSpotColor{PANTONE} {PANTONE647PC} {PANTONE\SpotSpace 647\SpotSpace PC} {1 0.56 0 0.23}
\AddSpotColor{PANTONE} {PANTONE648PC} {PANTONE\SpotSpace 648\SpotSpace PC} {1 0.62 0 0.52}
\AddSpotColor{PANTONE} {PANTONE649PC} {PANTONE\SpotSpace 649\SpotSpace PC} {0.1 0.04 0 0.01}
\AddSpotColor{PANTONE} {PANTONE650PC} {PANTONE\SpotSpace 650\SpotSpace PC} {0.24 0.09 0 0.02}
\AddSpotColor{PANTONE} {PANTONE651PC} {PANTONE\SpotSpace 651\SpotSpace PC} {0.38 0.18 0 0.06}
\AddSpotColor{PANTONE} {PANTONE652PC} {PANTONE\SpotSpace 652\SpotSpace PC} {0.5 0.25 0 0.1}
\AddSpotColor{PANTONE} {PANTONE653PC} {PANTONE\SpotSpace 653\SpotSpace PC} {1 0.62 0 0.2}
\AddSpotColor{PANTONE} {PANTONE654PC} {PANTONE\SpotSpace 654\SpotSpace PC} {1 0.67 0 0.38}
\AddSpotColor{PANTONE} {PANTONE655PC} {PANTONE\SpotSpace 655\SpotSpace PC} {1 0.68 0 0.52}
\AddSpotColor{PANTONE} {PANTONE656PC} {PANTONE\SpotSpace 656\SpotSpace PC} {0.14 0.03 0 0}
\AddSpotColor{PANTONE} {PANTONE657PC} {PANTONE\SpotSpace 657\SpotSpace PC} {0.24 0.07 0 0}
\AddSpotColor{PANTONE} {PANTONE658PC} {PANTONE\SpotSpace 658\SpotSpace PC} {0.3 0.15 0 0}
\AddSpotColor{PANTONE} {PANTONE659PC} {PANTONE\SpotSpace 659\SpotSpace PC} {0.55 0.3 0 0}
\AddSpotColor{PANTONE} {PANTONE660PC} {PANTONE\SpotSpace 660\SpotSpace PC} {0.9 0.57 0 0}
\AddSpotColor{PANTONE} {PANTONE661PC} {PANTONE\SpotSpace 661\SpotSpace PC} {1 0.69 0 0.09}
\AddSpotColor{PANTONE} {PANTONE662PC} {PANTONE\SpotSpace 662\SpotSpace PC} {1 0.71 0 0.18}
\AddSpotColor{PANTONE} {PANTONE663PC} {PANTONE\SpotSpace 663\SpotSpace PC} {0.07 0.06 0 0}
\AddSpotColor{PANTONE} {PANTONE664PC} {PANTONE\SpotSpace 664\SpotSpace PC} {0.11 0.09 0 0}
\AddSpotColor{PANTONE} {PANTONE665PC} {PANTONE\SpotSpace 665\SpotSpace PC} {0.2 0.17 0 0.02}
\AddSpotColor{PANTONE} {PANTONE666PC} {PANTONE\SpotSpace 666\SpotSpace PC} {0.31 0.3 0 0.07}
\AddSpotColor{PANTONE} {PANTONE667PC} {PANTONE\SpotSpace 667\SpotSpace PC} {0.52 0.49 0 0.14}
\AddSpotColor{PANTONE} {PANTONE668PC} {PANTONE\SpotSpace 668\SpotSpace PC} {0.65 0.64 0 0.3}
\AddSpotColor{PANTONE} {PANTONE669PC} {PANTONE\SpotSpace 669\SpotSpace PC} {0.76 0.78 0 0.47}
\AddSpotColor{PANTONE} {PANTONE670PC} {PANTONE\SpotSpace 670\SpotSpace PC} {0 0.13 0 0}
\AddSpotColor{PANTONE} {PANTONE671PC} {PANTONE\SpotSpace 671\SpotSpace PC} {0.01 0.2 0 0}
\AddSpotColor{PANTONE} {PANTONE672PC} {PANTONE\SpotSpace 672\SpotSpace PC} {0.03 0.34 0 0}
\AddSpotColor{PANTONE} {PANTONE673PC} {PANTONE\SpotSpace 673\SpotSpace PC} {0.06 0.49 0 0}
\AddSpotColor{PANTONE} {PANTONE674PC} {PANTONE\SpotSpace 674\SpotSpace PC} {0.09 0.67 0 0}
\AddSpotColor{PANTONE} {PANTONE675PC} {PANTONE\SpotSpace 675\SpotSpace PC} {0.17 1 0 0.03}
\AddSpotColor{PANTONE} {PANTONE676PC} {PANTONE\SpotSpace 676\SpotSpace PC} {0.06 1 0 0.22}
\AddSpotColor{PANTONE} {PANTONE677PC} {PANTONE\SpotSpace 677\SpotSpace PC} {0.02 0.13 0 0}
\AddSpotColor{PANTONE} {PANTONE678PC} {PANTONE\SpotSpace 678\SpotSpace PC} {0.03 0.21 0 0}
\AddSpotColor{PANTONE} {PANTONE679PC} {PANTONE\SpotSpace 679\SpotSpace PC} {0.05 0.27 0 0}
\AddSpotColor{PANTONE} {PANTONE680PC} {PANTONE\SpotSpace 680\SpotSpace PC} {0.1 0.43 0 0.02}
\AddSpotColor{PANTONE} {PANTONE681PC} {PANTONE\SpotSpace 681\SpotSpace PC} {0.21 0.61 0 0.04}
\AddSpotColor{PANTONE} {PANTONE682PC} {PANTONE\SpotSpace 682\SpotSpace PC} {0.25 0.79 0 0.12}
\AddSpotColor{PANTONE} {PANTONE683PC} {PANTONE\SpotSpace 683\SpotSpace PC} {0.11 1 0 0.43}
\AddSpotColor{PANTONE} {PANTONE684PC} {PANTONE\SpotSpace 684\SpotSpace PC} {0 0.17 0 0.02}
\AddSpotColor{PANTONE} {PANTONE685PC} {PANTONE\SpotSpace 685\SpotSpace PC} {0 0.25 0 0.03}
\AddSpotColor{PANTONE} {PANTONE686PC} {PANTONE\SpotSpace 686\SpotSpace PC} {0 0.3 0 0.05}
\AddSpotColor{PANTONE} {PANTONE687PC} {PANTONE\SpotSpace 687\SpotSpace PC} {0.02 0.44 0 0.12}
\AddSpotColor{PANTONE} {PANTONE688PC} {PANTONE\SpotSpace 688\SpotSpace PC} {0.05 0.57 0 0.19}
\AddSpotColor{PANTONE} {PANTONE689PC} {PANTONE\SpotSpace 689\SpotSpace PC} {0.07 0.77 0 0.34}
\AddSpotColor{PANTONE} {PANTONE690PC} {PANTONE\SpotSpace 690\SpotSpace PC} {0 0.97 0 0.59}
\AddSpotColor{PANTONE} {PANTONE691PC} {PANTONE\SpotSpace 691\SpotSpace PC} {0 0.15 0.08 0.01}
\AddSpotColor{PANTONE} {PANTONE692PC} {PANTONE\SpotSpace 692\SpotSpace PC} {0 0.23 0.1 0.02}
\AddSpotColor{PANTONE} {PANTONE693PC} {PANTONE\SpotSpace 693\SpotSpace PC} {0 0.3 0.12 0.06}
\AddSpotColor{PANTONE} {PANTONE694PC} {PANTONE\SpotSpace 694\SpotSpace PC} {0 0.36 0.21 0.1}
\AddSpotColor{PANTONE} {PANTONE695PC} {PANTONE\SpotSpace 695\SpotSpace PC} {0 0.5 0.28 0.2}
\AddSpotColor{PANTONE} {PANTONE696PC} {PANTONE\SpotSpace 696\SpotSpace PC} {0 0.6 0.36 0.32}
\AddSpotColor{PANTONE} {PANTONE697PC} {PANTONE\SpotSpace 697\SpotSpace PC} {0 0.68 0.47 0.42}
\AddSpotColor{PANTONE} {PANTONE698PC} {PANTONE\SpotSpace 698\SpotSpace PC} {0 0.16 0.08 0}
\AddSpotColor{PANTONE} {PANTONE699PC} {PANTONE\SpotSpace 699\SpotSpace PC} {0 0.24 0.1 0}
\AddSpotColor{PANTONE} {PANTONE700PC} {PANTONE\SpotSpace 700\SpotSpace PC} {0 0.36 0.14 0}
\AddSpotColor{PANTONE} {PANTONE701PC} {PANTONE\SpotSpace 701\SpotSpace PC} {0 0.45 0.2 0}
\AddSpotColor{PANTONE} {PANTONE702PC} {PANTONE\SpotSpace 702\SpotSpace PC} {0 0.69 0.34 0.05}
\AddSpotColor{PANTONE} {PANTONE703PC} {PANTONE\SpotSpace 703\SpotSpace PC} {0 0.83 0.54 0.16}
\AddSpotColor{PANTONE} {PANTONE704PC} {PANTONE\SpotSpace 704\SpotSpace PC} {0 0.9 0.72 0.29}
\AddSpotColor{PANTONE} {PANTONE705PC} {PANTONE\SpotSpace 705\SpotSpace PC} {0 0.09 0.06 0}
\AddSpotColor{PANTONE} {PANTONE706PC} {PANTONE\SpotSpace 706\SpotSpace PC} {0 0.17 0.1 0}
\AddSpotColor{PANTONE} {PANTONE707PC} {PANTONE\SpotSpace 707\SpotSpace PC} {0 0.3 0.14 0}
\AddSpotColor{PANTONE} {PANTONE708PC} {PANTONE\SpotSpace 708\SpotSpace PC} {0 0.46 0.22 0}
\AddSpotColor{PANTONE} {PANTONE709PC} {PANTONE\SpotSpace 709\SpotSpace PC} {0 0.66 0.38 0}
\AddSpotColor{PANTONE} {PANTONE710PC} {PANTONE\SpotSpace 710\SpotSpace PC} {0 0.79 0.58 0}
\AddSpotColor{PANTONE} {PANTONE711PC} {PANTONE\SpotSpace 711\SpotSpace PC} {0 1 0.8 0.02}
\AddSpotColor{PANTONE} {PANTONE712PC} {PANTONE\SpotSpace 712\SpotSpace PC} {0 0.14 0.31 0}
\AddSpotColor{PANTONE} {PANTONE713PC} {PANTONE\SpotSpace 713\SpotSpace PC} {0 0.19 0.41 0}
\AddSpotColor{PANTONE} {PANTONE714PC} {PANTONE\SpotSpace 714\SpotSpace PC} {0 0.27 0.55 0}
\AddSpotColor{PANTONE} {PANTONE715PC} {PANTONE\SpotSpace 715\SpotSpace PC} {0 0.36 0.71 0}
\AddSpotColor{PANTONE} {PANTONE716PC} {PANTONE\SpotSpace 716\SpotSpace PC} {0 0.45 0.91 0}
\AddSpotColor{PANTONE} {PANTONE717PC} {PANTONE\SpotSpace 717\SpotSpace PC} {0 0.53 1 0.02}
\AddSpotColor{PANTONE} {PANTONE718PC} {PANTONE\SpotSpace 718\SpotSpace PC} {0 0.56 1 0.08}
\AddSpotColor{PANTONE} {PANTONE719PC} {PANTONE\SpotSpace 719\SpotSpace PC} {0 0.1 0.25 0}
\AddSpotColor{PANTONE} {PANTONE720PC} {PANTONE\SpotSpace 720\SpotSpace PC} {0 0.15 0.36 0.01}
\AddSpotColor{PANTONE} {PANTONE721PC} {PANTONE\SpotSpace 721\SpotSpace PC} {0 0.24 0.52 0.03}
\AddSpotColor{PANTONE} {PANTONE722PC} {PANTONE\SpotSpace 722\SpotSpace PC} {0 0.36 0.76 0.09}
\AddSpotColor{PANTONE} {PANTONE723PC} {PANTONE\SpotSpace 723\SpotSpace PC} {0 0.43 0.97 0.17}
\AddSpotColor{PANTONE} {PANTONE724PC} {PANTONE\SpotSpace 724\SpotSpace PC} {0 0.51 1 0.36}
\AddSpotColor{PANTONE} {PANTONE725PC} {PANTONE\SpotSpace 725\SpotSpace PC} {0 0.53 1 0.48}
\AddSpotColor{PANTONE} {PANTONE726PC} {PANTONE\SpotSpace 726\SpotSpace PC} {0 0.08 0.23 0.02}
\AddSpotColor{PANTONE} {PANTONE727PC} {PANTONE\SpotSpace 727\SpotSpace PC} {0 0.15 0.34 0.05}
\AddSpotColor{PANTONE} {PANTONE728PC} {PANTONE\SpotSpace 728\SpotSpace PC} {0 0.21 0.48 0.1}
\AddSpotColor{PANTONE} {PANTONE729PC} {PANTONE\SpotSpace 729\SpotSpace PC} {0 0.31 0.62 0.18}
\AddSpotColor{PANTONE} {PANTONE730PC} {PANTONE\SpotSpace 730\SpotSpace PC} {0 0.38 0.78 0.29}
\AddSpotColor{PANTONE} {PANTONE731PC} {PANTONE\SpotSpace 731\SpotSpace PC} {0 0.52 1 0.54}
\AddSpotColor{PANTONE} {PANTONE732PC} {PANTONE\SpotSpace 732\SpotSpace PC} {0 0.55 1 0.64}
\AddSpotColor{PANTONE} {PANTONE1205PC} {PANTONE\SpotSpace 1205\SpotSpace PC} {0 0.05 0.31 0}
\AddSpotColor{PANTONE} {PANTONE1215PC} {PANTONE\SpotSpace 1215\SpotSpace PC} {0 0.09 0.45 0}
\AddSpotColor{PANTONE} {PANTONE1225PC} {PANTONE\SpotSpace 1225\SpotSpace PC} {0 0.17 0.62 0}
\AddSpotColor{PANTONE} {PANTONE1235PC} {PANTONE\SpotSpace 1235\SpotSpace PC} {0 0.29 0.91 0}
\AddSpotColor{PANTONE} {PANTONE1245PC} {PANTONE\SpotSpace 1245\SpotSpace PC} {0 0.28 1 0.18}
\AddSpotColor{PANTONE} {PANTONE1255PC} {PANTONE\SpotSpace 1255\SpotSpace PC} {0 0.27 1 0.34}
\AddSpotColor{PANTONE} {PANTONE1265PC} {PANTONE\SpotSpace 1265\SpotSpace PC} {0 0.27 1 0.51}
\AddSpotColor{PANTONE} {PANTONE1345PC} {PANTONE\SpotSpace 1345\SpotSpace PC} {0 0.14 0.47 0}
\AddSpotColor{PANTONE} {PANTONE1355PC} {PANTONE\SpotSpace 1355\SpotSpace PC} {0 0.2 0.56 0}
\AddSpotColor{PANTONE} {PANTONE1365PC} {PANTONE\SpotSpace 1365\SpotSpace PC} {0 0.29 0.72 0}
\AddSpotColor{PANTONE} {PANTONE1375PC} {PANTONE\SpotSpace 1375\SpotSpace PC} {0 0.4 0.9 0}
\AddSpotColor{PANTONE} {PANTONE1385PC} {PANTONE\SpotSpace 1385\SpotSpace PC} {0 0.44 1 0.07}
\AddSpotColor{PANTONE} {PANTONE1395PC} {PANTONE\SpotSpace 1395\SpotSpace PC} {0 0.41 1 0.37}
\AddSpotColor{PANTONE} {PANTONE1405PC} {PANTONE\SpotSpace 1405\SpotSpace PC} {0 0.36 1 0.63}
\AddSpotColor{PANTONE} {PANTONE1485PC} {PANTONE\SpotSpace 1485\SpotSpace PC} {0 0.27 0.54 0}
\AddSpotColor{PANTONE} {PANTONE1495PC} {PANTONE\SpotSpace 1495\SpotSpace PC} {0 0.33 0.67 0}
\AddSpotColor{PANTONE} {PANTONE1505PC} {PANTONE\SpotSpace 1505\SpotSpace PC} {0 0.42 0.77 0}
\AddSpotColor{PANTONE} {PANTONE1525PC} {PANTONE\SpotSpace 1525\SpotSpace PC} {0 0.58 1 0.1}
\AddSpotColor{PANTONE} {PANTONE1535PC} {PANTONE\SpotSpace 1535\SpotSpace PC} {0 0.53 1 0.38}
\AddSpotColor{PANTONE} {PANTONE1545PC} {PANTONE\SpotSpace 1545\SpotSpace PC} {0 0.53 1 0.72}
\AddSpotColor{PANTONE} {PANTONE1555PC} {PANTONE\SpotSpace 1555\SpotSpace PC} {0 0.22 0.34 0}
\AddSpotColor{PANTONE} {PANTONE1565PC} {PANTONE\SpotSpace 1565\SpotSpace PC} {0 0.34 0.49 0}
\AddSpotColor{PANTONE} {PANTONE1575PC} {PANTONE\SpotSpace 1575\SpotSpace PC} {0 0.45 0.72 0}
\AddSpotColor{PANTONE} {PANTONE1585PC} {PANTONE\SpotSpace 1585\SpotSpace PC} {0 0.56 0.9 0}
\AddSpotColor{PANTONE} {PANTONE1595PC} {PANTONE\SpotSpace 1595\SpotSpace PC} {0 0.59 1 0.05}
\AddSpotColor{PANTONE} {PANTONE1605PC} {PANTONE\SpotSpace 1605\SpotSpace PC} {0 0.56 1 0.3}
\AddSpotColor{PANTONE} {PANTONE1615PC} {PANTONE\SpotSpace 1615\SpotSpace PC} {0 0.56 1 0.43}
\AddSpotColor{PANTONE} {PANTONE1625PC} {PANTONE\SpotSpace 1625\SpotSpace PC} {0 0.31 0.37 0}
\AddSpotColor{PANTONE} {PANTONE1635PC} {PANTONE\SpotSpace 1635\SpotSpace PC} {0 0.39 0.48 0}
\AddSpotColor{PANTONE} {PANTONE1645PC} {PANTONE\SpotSpace 1645\SpotSpace PC} {0 0.49 0.66 0}
\AddSpotColor{PANTONE} {PANTONE1655PC} {PANTONE\SpotSpace 1655\SpotSpace PC} {0 0.63 0.91 0}
\AddSpotColor{PANTONE} {PANTONE1665PC} {PANTONE\SpotSpace 1665\SpotSpace PC} {0 0.68 1 0}
\AddSpotColor{PANTONE} {PANTONE1675PC} {PANTONE\SpotSpace 1675\SpotSpace PC} {0 0.67 1 0.28}
\AddSpotColor{PANTONE} {PANTONE1685PC} {PANTONE\SpotSpace 1685\SpotSpace PC} {0 0.68 1 0.44}
\AddSpotColor{PANTONE} {PANTONE1765PC} {PANTONE\SpotSpace 1765\SpotSpace PC} {0 0.38 0.21 0}
\AddSpotColor{PANTONE} {PANTONE1767PC} {PANTONE\SpotSpace 1767\SpotSpace PC} {0 0.27 0.12 0}
\AddSpotColor{PANTONE} {PANTONE1775PC} {PANTONE\SpotSpace 1775\SpotSpace PC} {0 0.47 0.29 0}
\AddSpotColor{PANTONE} {PANTONE1777PC} {PANTONE\SpotSpace 1777\SpotSpace PC} {0 0.58 0.36 0}
\AddSpotColor{PANTONE} {PANTONE1785PC} {PANTONE\SpotSpace 1785\SpotSpace PC} {0 0.67 0.5 0}
\AddSpotColor{PANTONE} {PANTONE1787PC} {PANTONE\SpotSpace 1787\SpotSpace PC} {0 0.76 0.6 0}
\AddSpotColor{PANTONE} {PANTONE1788PC} {PANTONE\SpotSpace 1788\SpotSpace PC} {0 0.84 0.88 0}
\AddSpotColor{PANTONE} {PANTONE1795PC} {PANTONE\SpotSpace 1795\SpotSpace PC} {0 0.94 1 0}
\AddSpotColor{PANTONE} {PANTONE1797PC} {PANTONE\SpotSpace 1797\SpotSpace PC} {0 1 0.99 0.04}
\AddSpotColor{PANTONE} {PANTONE1805PC} {PANTONE\SpotSpace 1805\SpotSpace PC} {0 0.91 1 0.23}
\AddSpotColor{PANTONE} {PANTONE1807PC} {PANTONE\SpotSpace 1807\SpotSpace PC} {0 1 0.96 0.28}
\AddSpotColor{PANTONE} {PANTONE1815PC} {PANTONE\SpotSpace 1815\SpotSpace PC} {0 0.9 1 0.51}
\AddSpotColor{PANTONE} {PANTONE1817PC} {PANTONE\SpotSpace 1817\SpotSpace PC} {0 0.9 1 0.66}
\AddSpotColor{PANTONE} {PANTONE1895PC} {PANTONE\SpotSpace 1895\SpotSpace PC} {0 0.28 0.07 0}
\AddSpotColor{PANTONE} {PANTONE1905PC} {PANTONE\SpotSpace 1905\SpotSpace PC} {0 0.41 0.09 0}
\AddSpotColor{PANTONE} {PANTONE1915PC} {PANTONE\SpotSpace 1915\SpotSpace PC} {0 0.71 0.2 0}
\AddSpotColor{PANTONE} {PANTONE1925PC} {PANTONE\SpotSpace 1925\SpotSpace PC} {0 1 0.55 0}
\AddSpotColor{PANTONE} {PANTONE1935PC} {PANTONE\SpotSpace 1935\SpotSpace PC} {0 1 0.57 0.05}
\AddSpotColor{PANTONE} {PANTONE1945PC} {PANTONE\SpotSpace 1945\SpotSpace PC} {0 1 0.56 0.19}
\AddSpotColor{PANTONE} {PANTONE1955PC} {PANTONE\SpotSpace 1955\SpotSpace PC} {0 1 0.6 0.37}
\AddSpotColor{PANTONE} {PANTONE2365PC} {PANTONE\SpotSpace 2365\SpotSpace PC} {0.02 0.27 0 0}
\AddSpotColor{PANTONE} {PANTONE2375PC} {PANTONE\SpotSpace 2375\SpotSpace PC} {0.1 0.57 0 0}
\AddSpotColor{PANTONE} {PANTONE2385PC} {PANTONE\SpotSpace 2385\SpotSpace PC} {0.19 0.79 0 0}
\AddSpotColor{PANTONE} {PANTONE2395PC} {PANTONE\SpotSpace 2395\SpotSpace PC} {0.27 0.95 0 0}
\AddSpotColor{PANTONE} {PANTONE2405PC} {PANTONE\SpotSpace 2405\SpotSpace PC} {0.34 1 0 0}
\AddSpotColor{PANTONE} {PANTONE2415PC} {PANTONE\SpotSpace 2415\SpotSpace PC} {0.33 1 0 0.08}
\AddSpotColor{PANTONE} {PANTONE2425PC} {PANTONE\SpotSpace 2425\SpotSpace PC} {0.37 1 0 0.26}
\AddSpotColor{PANTONE} {PANTONE2562PC} {PANTONE\SpotSpace 2562\SpotSpace PC} {0.19 0.35 0 0}
\AddSpotColor{PANTONE} {PANTONE2563PC} {PANTONE\SpotSpace 2563\SpotSpace PC} {0.22 0.33 0 0}
\AddSpotColor{PANTONE} {PANTONE2567PC} {PANTONE\SpotSpace 2567\SpotSpace PC} {0.29 0.36 0 0}
\AddSpotColor{PANTONE} {PANTONE2572PC} {PANTONE\SpotSpace 2572\SpotSpace PC} {0.3 0.47 0 0}
\AddSpotColor{PANTONE} {PANTONE2573PC} {PANTONE\SpotSpace 2573\SpotSpace PC} {0.3 0.43 0 0}
\AddSpotColor{PANTONE} {PANTONE2577PC} {PANTONE\SpotSpace 2577\SpotSpace PC} {0.4 0.45 0 0}
\AddSpotColor{PANTONE} {PANTONE2582PC} {PANTONE\SpotSpace 2582\SpotSpace PC} {0.46 0.72 0 0}
\AddSpotColor{PANTONE} {PANTONE2583PC} {PANTONE\SpotSpace 2583\SpotSpace PC} {0.46 0.63 0 0}
\AddSpotColor{PANTONE} {PANTONE2587PC} {PANTONE\SpotSpace 2587\SpotSpace PC} {0.59 0.66 0 0}
\AddSpotColor{PANTONE} {PANTONE2592PC} {PANTONE\SpotSpace 2592\SpotSpace PC} {0.6 0.9 0 0}
\AddSpotColor{PANTONE} {PANTONE2593PC} {PANTONE\SpotSpace 2593\SpotSpace PC} {0.61 0.89 0 0}
\AddSpotColor{PANTONE} {PANTONE2597PC} {PANTONE\SpotSpace 2597\SpotSpace PC} {0.85 1 0 0}
\AddSpotColor{PANTONE} {PANTONE2602PC} {PANTONE\SpotSpace 2602\SpotSpace PC} {0.63 1 0 0.03}
\AddSpotColor{PANTONE} {PANTONE2603PC} {PANTONE\SpotSpace 2603\SpotSpace PC} {0.69 1 0 0.02}
\AddSpotColor{PANTONE} {PANTONE2607PC} {PANTONE\SpotSpace 2607\SpotSpace PC} {0.81 1 0 0.07}
\AddSpotColor{PANTONE} {PANTONE2612PC} {PANTONE\SpotSpace 2612\SpotSpace PC} {0.64 1 0 0.14}
\AddSpotColor{PANTONE} {PANTONE2613PC} {PANTONE\SpotSpace 2613\SpotSpace PC} {0.63 1 0 0.15}
\AddSpotColor{PANTONE} {PANTONE2617PC} {PANTONE\SpotSpace 2617\SpotSpace PC} {0.79 1 0 0.15}
\AddSpotColor{PANTONE} {PANTONE2622PC} {PANTONE\SpotSpace 2622\SpotSpace PC} {0.57 0.98 0 0.46}
\AddSpotColor{PANTONE} {PANTONE2623PC} {PANTONE\SpotSpace 2623\SpotSpace PC} {0.59 1 0 0.32}
\AddSpotColor{PANTONE} {PANTONE2627PC} {PANTONE\SpotSpace 2627\SpotSpace PC} {0.77 1 0 0.31}
\AddSpotColor{PANTONE} {PANTONE2635PC} {PANTONE\SpotSpace 2635\SpotSpace PC} {0.28 0.27 0 0}
\AddSpotColor{PANTONE} {PANTONE2645PC} {PANTONE\SpotSpace 2645\SpotSpace PC} {0.4 0.36 0 0}
\AddSpotColor{PANTONE} {PANTONE2655PC} {PANTONE\SpotSpace 2655\SpotSpace PC} {0.54 0.49 0 0}
\AddSpotColor{PANTONE} {PANTONE2665PC} {PANTONE\SpotSpace 2665\SpotSpace PC} {0.62 0.6 0 0}
\AddSpotColor{PANTONE} {PANTONE2685PC} {PANTONE\SpotSpace 2685\SpotSpace PC} {0.96 1 0 0.1}
\AddSpotColor{PANTONE} {PANTONE2695PC} {PANTONE\SpotSpace 2695\SpotSpace PC} {0.91 1 0 0.49}
\AddSpotColor{PANTONE} {PANTONE2705PC} {PANTONE\SpotSpace 2705\SpotSpace PC} {0.4 0.3 0 0}
\AddSpotColor{PANTONE} {PANTONE2706PC} {PANTONE\SpotSpace 2706\SpotSpace PC} {0.19 0.09 0 0}
\AddSpotColor{PANTONE} {PANTONE2707PC} {PANTONE\SpotSpace 2707\SpotSpace PC} {0.17 0.06 0 0}
\AddSpotColor{PANTONE} {PANTONE2708PC} {PANTONE\SpotSpace 2708\SpotSpace PC} {0.26 0.1 0 0}
\AddSpotColor{PANTONE} {PANTONE2715PC} {PANTONE\SpotSpace 2715\SpotSpace PC} {0.57 0.45 0 0}
\AddSpotColor{PANTONE} {PANTONE2716PC} {PANTONE\SpotSpace 2716\SpotSpace PC} {0.45 0.29 0 0}
\AddSpotColor{PANTONE} {PANTONE2717PC} {PANTONE\SpotSpace 2717\SpotSpace PC} {0.29 0.12 0 0}
\AddSpotColor{PANTONE} {PANTONE2718PC} {PANTONE\SpotSpace 2718\SpotSpace PC} {0.67 0.41 0 0}
\AddSpotColor{PANTONE} {PANTONE2725PC} {PANTONE\SpotSpace 2725\SpotSpace PC} {0.77 0.68 0 0}
\AddSpotColor{PANTONE} {PANTONE2726PC} {PANTONE\SpotSpace 2726\SpotSpace PC} {0.79 0.66 0 0}
\AddSpotColor{PANTONE} {PANTONE2727PC} {PANTONE\SpotSpace 2727\SpotSpace PC} {0.71 0.42 0 0}
\AddSpotColor{PANTONE} {PANTONE2728PC} {PANTONE\SpotSpace 2728\SpotSpace PC} {0.96 0.69 0 0}
\AddSpotColor{PANTONE} {PANTONE2735PC} {PANTONE\SpotSpace 2735\SpotSpace PC} {1 0.95 0 0.03}
\AddSpotColor{PANTONE} {PANTONE2736PC} {PANTONE\SpotSpace 2736\SpotSpace PC} {1 0.91 0 0}
\AddSpotColor{PANTONE} {PANTONE2738PC} {PANTONE\SpotSpace 2738\SpotSpace PC} {1 0.87 0 0.02}
\AddSpotColor{PANTONE} {PANTONE2745PC} {PANTONE\SpotSpace 2745\SpotSpace PC} {1 0.95 0 0.15}
\AddSpotColor{PANTONE} {PANTONE2746PC} {PANTONE\SpotSpace 2746\SpotSpace PC} {1 0.92 0 0.1}
\AddSpotColor{PANTONE} {PANTONE2747PC} {PANTONE\SpotSpace 2747\SpotSpace PC} {1 0.85 0 0.13}
\AddSpotColor{PANTONE} {PANTONE2748PC} {PANTONE\SpotSpace 2748\SpotSpace PC} {1 0.88 0 0.14}
\AddSpotColor{PANTONE} {PANTONE2755PC} {PANTONE\SpotSpace 2755\SpotSpace PC} {1 0.97 0 0.3}
\AddSpotColor{PANTONE} {PANTONE2756PC} {PANTONE\SpotSpace 2756\SpotSpace PC} {1 0.94 0 0.29}
\AddSpotColor{PANTONE} {PANTONE2757PC} {PANTONE\SpotSpace 2757\SpotSpace PC} {1 0.82 0 0.3}
\AddSpotColor{PANTONE} {PANTONE2758PC} {PANTONE\SpotSpace 2758\SpotSpace PC} {1 0.8 0 0.26}
\AddSpotColor{PANTONE} {PANTONE2765PC} {PANTONE\SpotSpace 2765\SpotSpace PC} {1 0.97 0 0.45}
\AddSpotColor{PANTONE} {PANTONE2766PC} {PANTONE\SpotSpace 2766\SpotSpace PC} {1 0.94 0 0.47}
\AddSpotColor{PANTONE} {PANTONE2767PC} {PANTONE\SpotSpace 2767\SpotSpace PC} {1 0.78 0 0.54}
\AddSpotColor{PANTONE} {PANTONE2768PC} {PANTONE\SpotSpace 2768\SpotSpace PC} {1 0.78 0 0.44}
\AddSpotColor{PANTONE} {PANTONE2905PC} {PANTONE\SpotSpace 2905\SpotSpace PC} {0.41 0.02 0 0}
\AddSpotColor{PANTONE} {PANTONE2915PC} {PANTONE\SpotSpace 2915\SpotSpace PC} {0.59 0.07 0 0}
\AddSpotColor{PANTONE} {PANTONE2925PC} {PANTONE\SpotSpace 2925\SpotSpace PC} {0.85 0.24 0 0}
\AddSpotColor{PANTONE} {PANTONE2935PC} {PANTONE\SpotSpace 2935\SpotSpace PC} {1 0.46 0 0}
\AddSpotColor{PANTONE} {PANTONE2945PC} {PANTONE\SpotSpace 2945\SpotSpace PC} {1 0.45 0 0.14}
\AddSpotColor{PANTONE} {PANTONE2955PC} {PANTONE\SpotSpace 2955\SpotSpace PC} {1 0.45 0 0.37}
\AddSpotColor{PANTONE} {PANTONE2965PC} {PANTONE\SpotSpace 2965\SpotSpace PC} {1 0.38 0 0.64}
\AddSpotColor{PANTONE} {PANTONE2975PC} {PANTONE\SpotSpace 2975\SpotSpace PC} {0.3 0 0.05 0}
\AddSpotColor{PANTONE} {PANTONE2985PC} {PANTONE\SpotSpace 2985\SpotSpace PC} {0.59 0 0.06 0}
\AddSpotColor{PANTONE} {PANTONE2995PC} {PANTONE\SpotSpace 2995\SpotSpace PC} {0.9 0.11 0 0}
\AddSpotColor{PANTONE} {PANTONE3005PC} {PANTONE\SpotSpace 3005\SpotSpace PC} {1 0.34 0 0.02}
\AddSpotColor{PANTONE} {PANTONE3015PC} {PANTONE\SpotSpace 3015\SpotSpace PC} {1 0.3 0 0.2}
\AddSpotColor{PANTONE} {PANTONE3025PC} {PANTONE\SpotSpace 3025\SpotSpace PC} {1 0.17 0 0.51}
\AddSpotColor{PANTONE} {PANTONE3035PC} {PANTONE\SpotSpace 3035\SpotSpace PC} {1 0 0.05 0.72}
\AddSpotColor{PANTONE} {PANTONE3105PC} {PANTONE\SpotSpace 3105\SpotSpace PC} {0.43 0 0.12 0}
\AddSpotColor{PANTONE} {PANTONE3115PC} {PANTONE\SpotSpace 3115\SpotSpace PC} {0.63 0 0.18 0}
\AddSpotColor{PANTONE} {PANTONE3125PC} {PANTONE\SpotSpace 3125\SpotSpace PC} {0.83 0 0.21 0}
\AddSpotColor{PANTONE} {PANTONE3135PC} {PANTONE\SpotSpace 3135\SpotSpace PC} {1 0 0.16 0.09}
\AddSpotColor{PANTONE} {PANTONE3145PC} {PANTONE\SpotSpace 3145\SpotSpace PC} {1 0 0.19 0.23}
\AddSpotColor{PANTONE} {PANTONE3155PC} {PANTONE\SpotSpace 3155\SpotSpace PC} {1 0 0.24 0.38}
\AddSpotColor{PANTONE} {PANTONE3165PC} {PANTONE\SpotSpace 3165\SpotSpace PC} {1 0 0.28 0.65}
\AddSpotColor{PANTONE} {PANTONE3242PC} {PANTONE\SpotSpace 3242\SpotSpace PC} {0.37 0 0.18 0}
\AddSpotColor{PANTONE} {PANTONE3245PC} {PANTONE\SpotSpace 3245\SpotSpace PC} {0.34 0 0.19 0}
\AddSpotColor{PANTONE} {PANTONE3248PC} {PANTONE\SpotSpace 3248\SpotSpace PC} {0.43 0 0.24 0}
\AddSpotColor{PANTONE} {PANTONE3252PC} {PANTONE\SpotSpace 3252\SpotSpace PC} {0.47 0 0.24 0}
\AddSpotColor{PANTONE} {PANTONE3255PC} {PANTONE\SpotSpace 3255\SpotSpace PC} {0.49 0 0.28 0}
\AddSpotColor{PANTONE} {PANTONE3258PC} {PANTONE\SpotSpace 3258\SpotSpace PC} {0.59 0 0.33 0}
\AddSpotColor{PANTONE} {PANTONE3262PC} {PANTONE\SpotSpace 3262\SpotSpace PC} {0.71 0 0.33 0}
\AddSpotColor{PANTONE} {PANTONE3265PC} {PANTONE\SpotSpace 3265\SpotSpace PC} {0.69 0 0.37 0}
\AddSpotColor{PANTONE} {PANTONE3268PC} {PANTONE\SpotSpace 3268\SpotSpace PC} {0.9 0 0.49 0}
\AddSpotColor{PANTONE} {PANTONE3272PC} {PANTONE\SpotSpace 3272\SpotSpace PC} {1 0 0.44 0}
\AddSpotColor{PANTONE} {PANTONE3275PC} {PANTONE\SpotSpace 3275\SpotSpace PC} {0.95 0 0.47 0}
\AddSpotColor{PANTONE} {PANTONE3278PC} {PANTONE\SpotSpace 3278\SpotSpace PC} {1 0 0.55 0.05}
\AddSpotColor{PANTONE} {PANTONE3282PC} {PANTONE\SpotSpace 3282\SpotSpace PC} {1 0 0.46 0.15}
\AddSpotColor{PANTONE} {PANTONE3285PC} {PANTONE\SpotSpace 3285\SpotSpace PC} {1 0 0.5 0.07}
\AddSpotColor{PANTONE} {PANTONE3288PC} {PANTONE\SpotSpace 3288\SpotSpace PC} {1 0 0.54 0.2}
\AddSpotColor{PANTONE} {PANTONE3292PC} {PANTONE\SpotSpace 3292\SpotSpace PC} {1 0 0.49 0.46}
\AddSpotColor{PANTONE} {PANTONE3295PC} {PANTONE\SpotSpace 3295\SpotSpace PC} {1 0 0.53 0.21}
\AddSpotColor{PANTONE} {PANTONE3298PC} {PANTONE\SpotSpace 3298\SpotSpace PC} {1 0 0.57 0.42}
\AddSpotColor{PANTONE} {PANTONE3302PC} {PANTONE\SpotSpace 3302\SpotSpace PC} {1 0 0.54 0.69}
\AddSpotColor{PANTONE} {PANTONE3305PC} {PANTONE\SpotSpace 3305\SpotSpace PC} {1 0 0.61 0.61}
\AddSpotColor{PANTONE} {PANTONE3308PC} {PANTONE\SpotSpace 3308\SpotSpace PC} {1 0 0.6 0.72}
\AddSpotColor{PANTONE} {PANTONE3375PC} {PANTONE\SpotSpace 3375\SpotSpace PC} {0.35 0 0.25 0}
\AddSpotColor{PANTONE} {PANTONE3385PC} {PANTONE\SpotSpace 3385\SpotSpace PC} {0.45 0 0.33 0}
\AddSpotColor{PANTONE} {PANTONE3395PC} {PANTONE\SpotSpace 3395\SpotSpace PC} {0.61 0 0.45 0}
\AddSpotColor{PANTONE} {PANTONE3405PC} {PANTONE\SpotSpace 3405\SpotSpace PC} {0.85 0 0.65 0}
\AddSpotColor{PANTONE} {PANTONE3415PC} {PANTONE\SpotSpace 3415\SpotSpace PC} {1 0 0.77 0.22}
\AddSpotColor{PANTONE} {PANTONE3425PC} {PANTONE\SpotSpace 3425\SpotSpace PC} {1 0 0.78 0.42}
\AddSpotColor{PANTONE} {PANTONE3435PC} {PANTONE\SpotSpace 3435\SpotSpace PC} {1 0 0.81 0.66}
\AddSpotColor{PANTONE} {PANTONE3935PC} {PANTONE\SpotSpace 3935\SpotSpace PC} {0.01 0 0.68 0}
\AddSpotColor{PANTONE} {PANTONE3945PC} {PANTONE\SpotSpace 3945\SpotSpace PC} {0.03 0 0.85 0}
\AddSpotColor{PANTONE} {PANTONE3955PC} {PANTONE\SpotSpace 3955\SpotSpace PC} {0.06 0 1 0}
\AddSpotColor{PANTONE} {PANTONE3965PC} {PANTONE\SpotSpace 3965\SpotSpace PC} {0.08 0 1 0}
\AddSpotColor{PANTONE} {PANTONE3975PC} {PANTONE\SpotSpace 3975\SpotSpace PC} {0 0 1 0.29}
\AddSpotColor{PANTONE} {PANTONE3985PC} {PANTONE\SpotSpace 3985\SpotSpace PC} {0 0.03 1 0.41}
\AddSpotColor{PANTONE} {PANTONE3995PC} {PANTONE\SpotSpace 3995\SpotSpace PC} {0 0.03 1 0.64}
\AddSpotColor{PANTONE} {PANTONE4485PC} {PANTONE\SpotSpace 4485\SpotSpace PC} {0 0.26 1 0.69}
\AddSpotColor{PANTONE} {PANTONE4495PC} {PANTONE\SpotSpace 4495\SpotSpace PC} {0 0.2 0.95 0.46}
\AddSpotColor{PANTONE} {PANTONE4505PC} {PANTONE\SpotSpace 4505\SpotSpace PC} {0 0.15 0.78 0.36}
\AddSpotColor{PANTONE} {PANTONE4515PC} {PANTONE\SpotSpace 4515\SpotSpace PC} {0 0.09 0.5 0.24}
\AddSpotColor{PANTONE} {PANTONE4525PC} {PANTONE\SpotSpace 4525\SpotSpace PC} {0 0.07 0.39 0.17}
\AddSpotColor{PANTONE} {PANTONE4535PC} {PANTONE\SpotSpace 4535\SpotSpace PC} {0 0.04 0.3 0.11}
\AddSpotColor{PANTONE} {PANTONE4545PC} {PANTONE\SpotSpace 4545\SpotSpace PC} {0 0.03 0.19 0.06}
\AddSpotColor{PANTONE} {PANTONE4625PC} {PANTONE\SpotSpace 4625\SpotSpace PC} {0 0.6 1 0.79}
\AddSpotColor{PANTONE} {PANTONE4635PC} {PANTONE\SpotSpace 4635\SpotSpace PC} {0 0.48 0.96 0.44}
\AddSpotColor{PANTONE} {PANTONE4645PC} {PANTONE\SpotSpace 4645\SpotSpace PC} {0 0.37 0.68 0.28}
\AddSpotColor{PANTONE} {PANTONE4655PC} {PANTONE\SpotSpace 4655\SpotSpace PC} {0 0.26 0.45 0.18}
\AddSpotColor{PANTONE} {PANTONE4665PC} {PANTONE\SpotSpace 4665\SpotSpace PC} {0 0.18 0.32 0.1}
\AddSpotColor{PANTONE} {PANTONE4675PC} {PANTONE\SpotSpace 4675\SpotSpace PC} {0 0.11 0.21 0.06}
\AddSpotColor{PANTONE} {PANTONE4685PC} {PANTONE\SpotSpace 4685\SpotSpace PC} {0 0.07 0.14 0.04}
\AddSpotColor{PANTONE} {PANTONE4695PC} {PANTONE\SpotSpace 4695\SpotSpace PC} {0 0.81 1 0.77}
\AddSpotColor{PANTONE} {PANTONE4705PC} {PANTONE\SpotSpace 4705\SpotSpace PC} {0 0.62 0.71 0.49}
\AddSpotColor{PANTONE} {PANTONE4715PC} {PANTONE\SpotSpace 4715\SpotSpace PC} {0 0.42 0.45 0.34}
\AddSpotColor{PANTONE} {PANTONE4725PC} {PANTONE\SpotSpace 4725\SpotSpace PC} {0 0.32 0.35 0.25}
\AddSpotColor{PANTONE} {PANTONE4735PC} {PANTONE\SpotSpace 4735\SpotSpace PC} {0 0.22 0.23 0.15}
\AddSpotColor{PANTONE} {PANTONE4745PC} {PANTONE\SpotSpace 4745\SpotSpace PC} {0 0.17 0.18 0.1}
\AddSpotColor{PANTONE} {PANTONE4755PC} {PANTONE\SpotSpace 4755\SpotSpace PC} {0 0.1 0.12 0.06}
\AddSpotColor{PANTONE} {PANTONE4975PC} {PANTONE\SpotSpace 4975\SpotSpace PC} {0 0.73 1 0.8}
\AddSpotColor{PANTONE} {PANTONE4985PC} {PANTONE\SpotSpace 4985\SpotSpace PC} {0 0.59 0.48 0.48}
\AddSpotColor{PANTONE} {PANTONE4995PC} {PANTONE\SpotSpace 4995\SpotSpace PC} {0 0.48 0.38 0.34}
\AddSpotColor{PANTONE} {PANTONE5005PC} {PANTONE\SpotSpace 5005\SpotSpace PC} {0 0.38 0.27 0.23}
\AddSpotColor{PANTONE} {PANTONE5015PC} {PANTONE\SpotSpace 5015\SpotSpace PC} {0 0.25 0.15 0.11}
\AddSpotColor{PANTONE} {PANTONE5025PC} {PANTONE\SpotSpace 5025\SpotSpace PC} {0 0.18 0.12 0.07}
\AddSpotColor{PANTONE} {PANTONE5035PC} {PANTONE\SpotSpace 5035\SpotSpace PC} {0 0.1 0.09 0.03}
\AddSpotColor{PANTONE} {PANTONE5115PC} {PANTONE\SpotSpace 5115\SpotSpace PC} {0.75 1 0.7 0.15}
\AddSpotColor{PANTONE} {PANTONE5125PC} {PANTONE\SpotSpace 5125\SpotSpace PC} {0.65 0.86 0.49 0}
\AddSpotColor{PANTONE} {PANTONE5135PC} {PANTONE\SpotSpace 5135\SpotSpace PC} {0.47 0.64 0.28 0}
\AddSpotColor{PANTONE} {PANTONE5145PC} {PANTONE\SpotSpace 5145\SpotSpace PC} {0.3 0.44 0.13 0}
\AddSpotColor{PANTONE} {PANTONE5155PC} {PANTONE\SpotSpace 5155\SpotSpace PC} {0.17 0.29 0.08 0}
\AddSpotColor{PANTONE} {PANTONE5165PC} {PANTONE\SpotSpace 5165\SpotSpace PC} {0.08 0.17 0.05 0}
\AddSpotColor{PANTONE} {PANTONE5175PC} {PANTONE\SpotSpace 5175\SpotSpace PC} {0.05 0.1 0.03 0}
\AddSpotColor{PANTONE} {PANTONE5185PC} {PANTONE\SpotSpace 5185\SpotSpace PC} {0.8 1 0.85 0.25}
\AddSpotColor{PANTONE} {PANTONE5195PC} {PANTONE\SpotSpace 5195\SpotSpace PC} {0.72 0.9 0.75 0.15}
\AddSpotColor{PANTONE} {PANTONE5205PC} {PANTONE\SpotSpace 5205\SpotSpace PC} {0.5 0.58 0.5 0}
\AddSpotColor{PANTONE} {PANTONE5215PC} {PANTONE\SpotSpace 5215\SpotSpace PC} {0.28 0.35 0.24 0}
\AddSpotColor{PANTONE} {PANTONE5225PC} {PANTONE\SpotSpace 5225\SpotSpace PC} {0.17 0.25 0.15 0}
\AddSpotColor{PANTONE} {PANTONE5235PC} {PANTONE\SpotSpace 5235\SpotSpace PC} {0.1 0.15 0.1 0}
\AddSpotColor{PANTONE} {PANTONE5245PC} {PANTONE\SpotSpace 5245\SpotSpace PC} {0.06 0.08 0.07 0}
\AddSpotColor{PANTONE} {PANTONE5255PC} {PANTONE\SpotSpace 5255\SpotSpace PC} {1 0.8 0 0.55}
\AddSpotColor{PANTONE} {PANTONE5265PC} {PANTONE\SpotSpace 5265\SpotSpace PC} {0.77 0.7 0 0.4}
\AddSpotColor{PANTONE} {PANTONE5275PC} {PANTONE\SpotSpace 5275\SpotSpace PC} {0.6 0.47 0 0.3}
\AddSpotColor{PANTONE} {PANTONE5285PC} {PANTONE\SpotSpace 5285\SpotSpace PC} {0.31 0.27 0 0.2}
\AddSpotColor{PANTONE} {PANTONE5295PC} {PANTONE\SpotSpace 5295\SpotSpace PC} {0.2 0.15 0 0.1}
\AddSpotColor{PANTONE} {PANTONE5305PC} {PANTONE\SpotSpace 5305\SpotSpace PC} {0.14 0.1 0 0.06}
\AddSpotColor{PANTONE} {PANTONE5315PC} {PANTONE\SpotSpace 5315\SpotSpace PC} {0.06 0.06 0 0.05}
\AddSpotColor{PANTONE} {PANTONE5395PC} {PANTONE\SpotSpace 5395\SpotSpace PC} {1 0.44 0 0.76}
\AddSpotColor{PANTONE} {PANTONE5405PC} {PANTONE\SpotSpace 5405\SpotSpace PC} {0.58 0.17 0 0.46}
\AddSpotColor{PANTONE} {PANTONE5415PC} {PANTONE\SpotSpace 5415\SpotSpace PC} {0.42 0.08 0 0.4}
\AddSpotColor{PANTONE} {PANTONE5425PC} {PANTONE\SpotSpace 5425\SpotSpace PC} {0.3 0.04 0 0.31}
\AddSpotColor{PANTONE} {PANTONE5435PC} {PANTONE\SpotSpace 5435\SpotSpace PC} {0.13 0.03 0 0.17}
\AddSpotColor{PANTONE} {PANTONE5445PC} {PANTONE\SpotSpace 5445\SpotSpace PC} {0.08 0.01 0 0.13}
\AddSpotColor{PANTONE} {PANTONE5455PC} {PANTONE\SpotSpace 5455\SpotSpace PC} {0.06 0 0 0.09}
\AddSpotColor{PANTONE} {PANTONE5463PC} {PANTONE\SpotSpace 5463\SpotSpace PC} {1 0 0.18 0.83}
\AddSpotColor{PANTONE} {PANTONE5467PC} {PANTONE\SpotSpace 5467\SpotSpace PC} {1 0 0.33 0.94}
\AddSpotColor{PANTONE} {PANTONE5473PC} {PANTONE\SpotSpace 5473\SpotSpace PC} {0.82 0 0.28 0.52}
\AddSpotColor{PANTONE} {PANTONE5477PC} {PANTONE\SpotSpace 5477\SpotSpace PC} {0.55 0 0.27 0.73}
\AddSpotColor{PANTONE} {PANTONE5483PC} {PANTONE\SpotSpace 5483\SpotSpace PC} {0.62 0 0.21 0.31}
\AddSpotColor{PANTONE} {PANTONE5487PC} {PANTONE\SpotSpace 5487\SpotSpace PC} {0.35 0 0.16 0.54}
\AddSpotColor{PANTONE} {PANTONE5493PC} {PANTONE\SpotSpace 5493\SpotSpace PC} {0.43 0 0.14 0.21}
\AddSpotColor{PANTONE} {PANTONE5497PC} {PANTONE\SpotSpace 5497\SpotSpace PC} {0.17 0 0.09 0.63}
\AddSpotColor{PANTONE} {PANTONE5503PC} {PANTONE\SpotSpace 5503\SpotSpace PC} {0.29 0 0.1 0.14}
\AddSpotColor{PANTONE} {PANTONE5507PC} {PANTONE\SpotSpace 5507\SpotSpace PC} {0.1 0 0.06 0.27}
\AddSpotColor{PANTONE} {PANTONE5513PC} {PANTONE\SpotSpace 5513\SpotSpace PC} {0.18 0 0.07 0.05}
\AddSpotColor{PANTONE} {PANTONE5517PC} {PANTONE\SpotSpace 5517\SpotSpace PC} {0.08 0 0.05 0.17}
\AddSpotColor{PANTONE} {PANTONE5523PC} {PANTONE\SpotSpace 5523\SpotSpace PC} {0.11 0 0.05 0.03}
\AddSpotColor{PANTONE} {PANTONE5527PC} {PANTONE\SpotSpace 5527\SpotSpace PC} {0.06 0 0.04 0.11}
\AddSpotColor{PANTONE} {PANTONE5535PC} {PANTONE\SpotSpace 5535\SpotSpace PC} {0.66 0 0.57 0.82}
\AddSpotColor{PANTONE} {PANTONE5545PC} {PANTONE\SpotSpace 5545\SpotSpace PC} {0.59 0 0.5 0.52}
\AddSpotColor{PANTONE} {PANTONE5555PC} {PANTONE\SpotSpace 5555\SpotSpace PC} {0.43 0 0.34 0.38}
\AddSpotColor{PANTONE} {PANTONE5565PC} {PANTONE\SpotSpace 5565\SpotSpace PC} {0.3 0 0.24 0.26}
\AddSpotColor{PANTONE} {PANTONE5575PC} {PANTONE\SpotSpace 5575\SpotSpace PC} {0.2 0 0.16 0.17}
\AddSpotColor{PANTONE} {PANTONE5585PC} {PANTONE\SpotSpace 5585\SpotSpace PC} {0.12 0 0.11 0.1}
\AddSpotColor{PANTONE} {PANTONE5595PC} {PANTONE\SpotSpace 5595\SpotSpace PC} {0.07 0 0.08 0.07}
\AddSpotColor{PANTONE} {PANTONE5605PC} {PANTONE\SpotSpace 5605\SpotSpace PC} {0.65 0 0.56 0.94}
\AddSpotColor{PANTONE} {PANTONE5615PC} {PANTONE\SpotSpace 5615\SpotSpace PC} {0.49 0 0.44 0.64}
\AddSpotColor{PANTONE} {PANTONE5625PC} {PANTONE\SpotSpace 5625\SpotSpace PC} {0.28 0 0.29 0.48}
\AddSpotColor{PANTONE} {PANTONE5635PC} {PANTONE\SpotSpace 5635\SpotSpace PC} {0.13 0 0.18 0.33}
\AddSpotColor{PANTONE} {PANTONE5645PC} {PANTONE\SpotSpace 5645\SpotSpace PC} {0.07 0 0.11 0.23}
\AddSpotColor{PANTONE} {PANTONE5655PC} {PANTONE\SpotSpace 5655\SpotSpace PC} {0.06 0 0.09 0.16}
\AddSpotColor{PANTONE} {PANTONE5665PC} {PANTONE\SpotSpace 5665\SpotSpace PC} {0.05 0 0.07 0.1}
\AddSpotColor{PANTONE} {PANTONE5743PC} {PANTONE\SpotSpace 5743\SpotSpace PC} {0.33 0 0.85 0.82}
\AddSpotColor{PANTONE} {PANTONE5747PC} {PANTONE\SpotSpace 5747\SpotSpace PC} {0.32 0 1 0.79}
\AddSpotColor{PANTONE} {PANTONE5753PC} {PANTONE\SpotSpace 5753\SpotSpace PC} {0.25 0 0.81 0.67}
\AddSpotColor{PANTONE} {PANTONE5757PC} {PANTONE\SpotSpace 5757\SpotSpace PC} {0.27 0 0.95 0.55}
\AddSpotColor{PANTONE} {PANTONE5763PC} {PANTONE\SpotSpace 5763\SpotSpace PC} {0.16 0 0.74 0.57}
\AddSpotColor{PANTONE} {PANTONE5767PC} {PANTONE\SpotSpace 5767\SpotSpace PC} {0.15 0 0.68 0.39}
\AddSpotColor{PANTONE} {PANTONE5773PC} {PANTONE\SpotSpace 5773\SpotSpace PC} {0.09 0 0.43 0.38}
\AddSpotColor{PANTONE} {PANTONE5777PC} {PANTONE\SpotSpace 5777\SpotSpace PC} {0.1 0 0.49 0.28}
\AddSpotColor{PANTONE} {PANTONE5783PC} {PANTONE\SpotSpace 5783\SpotSpace PC} {0.06 0 0.28 0.27}
\AddSpotColor{PANTONE} {PANTONE5787PC} {PANTONE\SpotSpace 5787\SpotSpace PC} {0.07 0 0.31 0.13}
\AddSpotColor{PANTONE} {PANTONE5793PC} {PANTONE\SpotSpace 5793\SpotSpace PC} {0.04 0 0.21 0.18}
\AddSpotColor{PANTONE} {PANTONE5797PC} {PANTONE\SpotSpace 5797\SpotSpace PC} {0.05 0 0.24 0.09}
\AddSpotColor{PANTONE} {PANTONE5803PC} {PANTONE\SpotSpace 5803\SpotSpace PC} {0.02 0 0.12 0.11}
\AddSpotColor{PANTONE} {PANTONE5807PC} {PANTONE\SpotSpace 5807\SpotSpace PC} {0.02 0 0.14 0.03}
\AddSpotColor{PANTONE} {PANTONE5815PC} {PANTONE\SpotSpace 5815\SpotSpace PC} {0 0 0.91 0.79}
\AddSpotColor{PANTONE} {PANTONE5825PC} {PANTONE\SpotSpace 5825\SpotSpace PC} {0 0.02 0.87 0.59}
\AddSpotColor{PANTONE} {PANTONE5835PC} {PANTONE\SpotSpace 5835\SpotSpace PC} {0 0.02 0.67 0.4}
\AddSpotColor{PANTONE} {PANTONE5845PC} {PANTONE\SpotSpace 5845\SpotSpace PC} {0 0.01 0.47 0.3}
\AddSpotColor{PANTONE} {PANTONE5855PC} {PANTONE\SpotSpace 5855\SpotSpace PC} {0 0 0.31 0.18}
\AddSpotColor{PANTONE} {PANTONE5865PC} {PANTONE\SpotSpace 5865\SpotSpace PC} {0 0 0.25 0.13}
\AddSpotColor{PANTONE} {PANTONE5875PC} {PANTONE\SpotSpace 5875\SpotSpace PC} {0 0 0.26 0.11}
\AddSpotColor{PANTONE} {PANTONE7401PC} {PANTONE\SpotSpace 7401\SpotSpace PC} {0 0.04 0.18 0}
\AddSpotColor{PANTONE} {PANTONE7402PC} {PANTONE\SpotSpace 7402\SpotSpace PC} {0 0.06 0.3 0}
\AddSpotColor{PANTONE} {PANTONE7403PC} {PANTONE\SpotSpace 7403\SpotSpace PC} {0 0.1 0.5 0}
\AddSpotColor{PANTONE} {PANTONE7404PC} {PANTONE\SpotSpace 7404\SpotSpace PC} {0 0.09 0.79 0}
\AddSpotColor{PANTONE} {PANTONE7405PC} {PANTONE\SpotSpace 7405\SpotSpace PC} {0 0.1 0.99 0}
\AddSpotColor{PANTONE} {PANTONE7406PC} {PANTONE\SpotSpace 7406\SpotSpace PC} {0 0.18 1 0}
\AddSpotColor{PANTONE} {PANTONE7407PC} {PANTONE\SpotSpace 7407\SpotSpace PC} {0 0.22 0.85 0.11}
\AddSpotColor{PANTONE} {PANTONE7408PC} {PANTONE\SpotSpace 7408\SpotSpace PC} {0 0.25 0.95 0}
\AddSpotColor{PANTONE} {PANTONE7409PC} {PANTONE\SpotSpace 7409\SpotSpace PC} {0 0.3 0.95 0}
\AddSpotColor{PANTONE} {PANTONE7410PC} {PANTONE\SpotSpace 7410\SpotSpace PC} {0 0.3 0.55 0}
\AddSpotColor{PANTONE} {PANTONE7411PC} {PANTONE\SpotSpace 7411\SpotSpace PC} {0 0.35 0.69 0}
\AddSpotColor{PANTONE} {PANTONE7412PC} {PANTONE\SpotSpace 7412\SpotSpace PC} {0 0.42 1 0.07}
\AddSpotColor{PANTONE} {PANTONE7413PC} {PANTONE\SpotSpace 7413\SpotSpace PC} {0 0.53 1 0.04}
\AddSpotColor{PANTONE} {PANTONE7414PC} {PANTONE\SpotSpace 7414\SpotSpace PC} {0 0.46 1 0.11}
\AddSpotColor{PANTONE} {PANTONE7415PC} {PANTONE\SpotSpace 7415\SpotSpace PC} {0 0.18 0.15 0}
\AddSpotColor{PANTONE} {PANTONE7416PC} {PANTONE\SpotSpace 7416\SpotSpace PC} {0 0.6 0.6 0}
\AddSpotColor{PANTONE} {PANTONE7417PC} {PANTONE\SpotSpace 7417\SpotSpace PC} {0 0.75 0.75 0}
\AddSpotColor{PANTONE} {PANTONE7418PC} {PANTONE\SpotSpace 7418\SpotSpace PC} {0 0.7 0.6 0.05}
\AddSpotColor{PANTONE} {PANTONE7419PC} {PANTONE\SpotSpace 7419\SpotSpace PC} {0 0.6 0.45 0.18}
\AddSpotColor{PANTONE} {PANTONE7420PC} {PANTONE\SpotSpace 7420\SpotSpace PC} {0 0.8 0.42 0.2}
\AddSpotColor{PANTONE} {PANTONE7421PC} {PANTONE\SpotSpace 7421\SpotSpace PC} {0 1 0.3 0.61}
\AddSpotColor{PANTONE} {PANTONE7422PC} {PANTONE\SpotSpace 7422\SpotSpace PC} {0 0.09 0.05 0}
\AddSpotColor{PANTONE} {PANTONE7423PC} {PANTONE\SpotSpace 7423\SpotSpace PC} {0 0.55 0.23 0}
\AddSpotColor{PANTONE} {PANTONE7424PC} {PANTONE\SpotSpace 7424\SpotSpace PC} {0 0.75 0.3 0}
\AddSpotColor{PANTONE} {PANTONE7425PC} {PANTONE\SpotSpace 7425\SpotSpace PC} {0 0.9 0.3 0.07}
\AddSpotColor{PANTONE} {PANTONE7426PC} {PANTONE\SpotSpace 7426\SpotSpace PC} {0 1 0.45 0.18}
\AddSpotColor{PANTONE} {PANTONE7427PC} {PANTONE\SpotSpace 7427\SpotSpace PC} {0 1 0.65 0.28}
\AddSpotColor{PANTONE} {PANTONE7428PC} {PANTONE\SpotSpace 7428\SpotSpace PC} {0 0.8 0.45 0.55}
\AddSpotColor{PANTONE} {PANTONE7429PC} {PANTONE\SpotSpace 7429\SpotSpace PC} {0 0.18 0.03 0}
\AddSpotColor{PANTONE} {PANTONE7430PC} {PANTONE\SpotSpace 7430\SpotSpace PC} {0.02 0.31 0 0}
\AddSpotColor{PANTONE} {PANTONE7431PC} {PANTONE\SpotSpace 7431\SpotSpace PC} {0 0.38 0.02 0.05}
\AddSpotColor{PANTONE} {PANTONE7432PC} {PANTONE\SpotSpace 7432\SpotSpace PC} {0 0.55 0.03 0.1}
\AddSpotColor{PANTONE} {PANTONE7433PC} {PANTONE\SpotSpace 7433\SpotSpace PC} {0 0.75 0.15 0.15}
\AddSpotColor{PANTONE} {PANTONE7434PC} {PANTONE\SpotSpace 7434\SpotSpace PC} {0 0.8 0.15 0.2}
\AddSpotColor{PANTONE} {PANTONE7435PC} {PANTONE\SpotSpace 7435\SpotSpace PC} {0 1 0.1 0.35}
\AddSpotColor{PANTONE} {PANTONE7436PC} {PANTONE\SpotSpace 7436\SpotSpace PC} {0.03 0.08 0 0}
\AddSpotColor{PANTONE} {PANTONE7437PC} {PANTONE\SpotSpace 7437\SpotSpace PC} {0.06 0.2 0 0}
\AddSpotColor{PANTONE} {PANTONE7438PC} {PANTONE\SpotSpace 7438\SpotSpace PC} {0.15 0.35 0 0}
\AddSpotColor{PANTONE} {PANTONE7439PC} {PANTONE\SpotSpace 7439\SpotSpace PC} {0.2 0.35 0 0}
\AddSpotColor{PANTONE} {PANTONE7440PC} {PANTONE\SpotSpace 7440\SpotSpace PC} {0.3 0.4 0 0}
\AddSpotColor{PANTONE} {PANTONE7441PC} {PANTONE\SpotSpace 7441\SpotSpace PC} {0.36 0.5 0 0}
\AddSpotColor{PANTONE} {PANTONE7442PC} {PANTONE\SpotSpace 7442\SpotSpace PC} {0.5 0.7 0 0}
\AddSpotColor{PANTONE} {PANTONE7443PC} {PANTONE\SpotSpace 7443\SpotSpace PC} {0.06 0.05 0 0}
\AddSpotColor{PANTONE} {PANTONE7444PC} {PANTONE\SpotSpace 7444\SpotSpace PC} {0.2 0.17 0 0}
\AddSpotColor{PANTONE} {PANTONE7445PC} {PANTONE\SpotSpace 7445\SpotSpace PC} {0.3 0.2 0 0.03}
\AddSpotColor{PANTONE} {PANTONE7446PC} {PANTONE\SpotSpace 7446\SpotSpace PC} {0.43 0.38 0 0}
\AddSpotColor{PANTONE} {PANTONE7447PC} {PANTONE\SpotSpace 7447\SpotSpace PC} {0.6 0.58 0 0.19}
\AddSpotColor{PANTONE} {PANTONE7448PC} {PANTONE\SpotSpace 7448\SpotSpace PC} {0.32 0.42 0 0.55}
\AddSpotColor{PANTONE} {PANTONE7449PC} {PANTONE\SpotSpace 7449\SpotSpace PC} {0.72 1 0.77 0.4}
\AddSpotColor{PANTONE} {PANTONE7450PC} {PANTONE\SpotSpace 7450\SpotSpace PC} {0.2 0.1 0 0}
\AddSpotColor{PANTONE} {PANTONE7451PC} {PANTONE\SpotSpace 7451\SpotSpace PC} {0.4 0.21 0 0}
\AddSpotColor{PANTONE} {PANTONE7452PC} {PANTONE\SpotSpace 7452\SpotSpace PC} {0.5 0.32 0 0}
\AddSpotColor{PANTONE} {PANTONE7453PC} {PANTONE\SpotSpace 7453\SpotSpace PC} {0.5 0.26 0 0}
\AddSpotColor{PANTONE} {PANTONE7454PC} {PANTONE\SpotSpace 7454\SpotSpace PC} {0.5 0.24 0 0.1}
\AddSpotColor{PANTONE} {PANTONE7455PC} {PANTONE\SpotSpace 7455\SpotSpace PC} {0.8 0.53 0 0}
\AddSpotColor{PANTONE} {PANTONE7456PC} {PANTONE\SpotSpace 7456\SpotSpace PC} {0.55 0.35 0 0.07}
\AddSpotColor{PANTONE} {PANTONE7457PC} {PANTONE\SpotSpace 7457\SpotSpace PC} {0.12 0 0.02 0}
\AddSpotColor{PANTONE} {PANTONE7458PC} {PANTONE\SpotSpace 7458\SpotSpace PC} {0.4 0 0.05 0.06}
\AddSpotColor{PANTONE} {PANTONE7459PC} {PANTONE\SpotSpace 7459\SpotSpace PC} {0.57 0 0.06 0.13}
\AddSpotColor{PANTONE} {PANTONE7460PC} {PANTONE\SpotSpace 7460\SpotSpace PC} {1 0 0 0.05}
\AddSpotColor{PANTONE} {PANTONE7461PC} {PANTONE\SpotSpace 7461\SpotSpace PC} {0.78 0.28 0 0}
\AddSpotColor{PANTONE} {PANTONE7462PC} {PANTONE\SpotSpace 7462\SpotSpace PC} {1 0.5 0 0.1}
\AddSpotColor{PANTONE} {PANTONE7463PC} {PANTONE\SpotSpace 7463\SpotSpace PC} {1 0.43 0 0.65}
\AddSpotColor{PANTONE} {PANTONE7464PC} {PANTONE\SpotSpace 7464\SpotSpace PC} {0.25 0 0.1 0}
\AddSpotColor{PANTONE} {PANTONE7465PC} {PANTONE\SpotSpace 7465\SpotSpace PC} {0.5 0 0.25 0}
\AddSpotColor{PANTONE} {PANTONE7466PC} {PANTONE\SpotSpace 7466\SpotSpace PC} {0.7 0 0.23 0}
\AddSpotColor{PANTONE} {PANTONE7467PC} {PANTONE\SpotSpace 7467\SpotSpace PC} {0.95 0 0.25 0}
\AddSpotColor{PANTONE} {PANTONE7468PC} {PANTONE\SpotSpace 7468\SpotSpace PC} {1 0.1 0 0.28}
\AddSpotColor{PANTONE} {PANTONE7469PC} {PANTONE\SpotSpace 7469\SpotSpace PC} {1 0.2 0 0.4}
\AddSpotColor{PANTONE} {PANTONE7470PC} {PANTONE\SpotSpace 7470\SpotSpace PC} {0.8 0.15 0 0.45}
\AddSpotColor{PANTONE} {PANTONE7471PC} {PANTONE\SpotSpace 7471\SpotSpace PC} {0.28 0 0.14 0}
\AddSpotColor{PANTONE} {PANTONE7472PC} {PANTONE\SpotSpace 7472\SpotSpace PC} {0.52 0 0.25 0}
\AddSpotColor{PANTONE} {PANTONE7473PC} {PANTONE\SpotSpace 7473\SpotSpace PC} {0.7 0 0.38 0.08}
\AddSpotColor{PANTONE} {PANTONE7474PC} {PANTONE\SpotSpace 7474\SpotSpace PC} {0.9 0 0.28 0.22}
\AddSpotColor{PANTONE} {PANTONE7475PC} {PANTONE\SpotSpace 7475\SpotSpace PC} {0.5 0 0.25 0.3}
\AddSpotColor{PANTONE} {PANTONE7476PC} {PANTONE\SpotSpace 7476\SpotSpace PC} {1 0 0.43 0.6}
\AddSpotColor{PANTONE} {PANTONE7477PC} {PANTONE\SpotSpace 7477\SpotSpace PC} {0.8 0 0.1 0.68}
\AddSpotColor{PANTONE} {PANTONE7478PC} {PANTONE\SpotSpace 7478\SpotSpace PC} {0.18 0 0.14 0}
\AddSpotColor{PANTONE} {PANTONE7479PC} {PANTONE\SpotSpace 7479\SpotSpace PC} {0.55 0 0.5 0}
\AddSpotColor{PANTONE} {PANTONE7480PC} {PANTONE\SpotSpace 7480\SpotSpace PC} {0.6 0 0.5 0}
\AddSpotColor{PANTONE} {PANTONE7481PC} {PANTONE\SpotSpace 7481\SpotSpace PC} {0.6 0 0.55 0}
\AddSpotColor{PANTONE} {PANTONE7482PC} {PANTONE\SpotSpace 7482\SpotSpace PC} {0.8 0 0.75 0}
\AddSpotColor{PANTONE} {PANTONE7483PC} {PANTONE\SpotSpace 7483\SpotSpace PC} {0.85 0 1 0.55}
\AddSpotColor{PANTONE} {PANTONE7484PC} {PANTONE\SpotSpace 7484\SpotSpace PC} {1 0 0.85 0.5}
\AddSpotColor{PANTONE} {PANTONE7485PC} {PANTONE\SpotSpace 7485\SpotSpace PC} {0.06 0 0.1 0}
\AddSpotColor{PANTONE} {PANTONE7486PC} {PANTONE\SpotSpace 7486\SpotSpace PC} {0.2 0 0.3 0}
\AddSpotColor{PANTONE} {PANTONE7487PC} {PANTONE\SpotSpace 7487\SpotSpace PC} {0.3 0 0.45 0}
\AddSpotColor{PANTONE} {PANTONE7488PC} {PANTONE\SpotSpace 7488\SpotSpace PC} {0.43 0 0.6 0}
\AddSpotColor{PANTONE} {PANTONE7489PC} {PANTONE\SpotSpace 7489\SpotSpace PC} {0.6 0 0.8 0.07}
\AddSpotColor{PANTONE} {PANTONE7490PC} {PANTONE\SpotSpace 7490\SpotSpace PC} {0.45 0 0.8 0.35}
\AddSpotColor{PANTONE} {PANTONE7491PC} {PANTONE\SpotSpace 7491\SpotSpace PC} {0.32 0 1 0.4}
\AddSpotColor{PANTONE} {PANTONE7492PC} {PANTONE\SpotSpace 7492\SpotSpace PC} {0.12 0 0.5 0.07}
\AddSpotColor{PANTONE} {PANTONE7493PC} {PANTONE\SpotSpace 7493\SpotSpace PC} {0.14 0 0.36 0.1}
\AddSpotColor{PANTONE} {PANTONE7494PC} {PANTONE\SpotSpace 7494\SpotSpace PC} {0.25 0 0.4 0.15}
\AddSpotColor{PANTONE} {PANTONE7495PC} {PANTONE\SpotSpace 7495\SpotSpace PC} {0.25 0 0.8 0.3}
\AddSpotColor{PANTONE} {PANTONE7496PC} {PANTONE\SpotSpace 7496\SpotSpace PC} {0.4 0 1 0.38}
\AddSpotColor{PANTONE} {PANTONE7497PC} {PANTONE\SpotSpace 7497\SpotSpace PC} {0.4 0.3 0.7 0.25}
\AddSpotColor{PANTONE} {PANTONE7498PC} {PANTONE\SpotSpace 7498\SpotSpace PC} {0.25 0 1 0.8}
\AddSpotColor{PANTONE} {PANTONE7499PC} {PANTONE\SpotSpace 7499\SpotSpace PC} {0 0.02 0.15 0}
\AddSpotColor{PANTONE} {PANTONE7500PC} {PANTONE\SpotSpace 7500\SpotSpace PC} {0 0.02 0.15 0.03}
\AddSpotColor{PANTONE} {PANTONE7501PC} {PANTONE\SpotSpace 7501\SpotSpace PC} {0 0.04 0.2 0.06}
\AddSpotColor{PANTONE} {PANTONE7502PC} {PANTONE\SpotSpace 7502\SpotSpace PC} {0 0.08 0.35 0.1}
\AddSpotColor{PANTONE} {PANTONE7503PC} {PANTONE\SpotSpace 7503\SpotSpace PC} {0 0.12 0.35 0.25}
\AddSpotColor{PANTONE} {PANTONE7504PC} {PANTONE\SpotSpace 7504\SpotSpace PC} {0 0.25 0.45 0.4}
\AddSpotColor{PANTONE} {PANTONE7505PC} {PANTONE\SpotSpace 7505\SpotSpace PC} {0 0.3 0.7 0.55}
\AddSpotColor{PANTONE} {PANTONE7506PC} {PANTONE\SpotSpace 7506\SpotSpace PC} {0 0.05 0.15 0}
\AddSpotColor{PANTONE} {PANTONE7507PC} {PANTONE\SpotSpace 7507\SpotSpace PC} {0 0.1 0.3 0}
\AddSpotColor{PANTONE} {PANTONE7508PC} {PANTONE\SpotSpace 7508\SpotSpace PC} {0 0.15 0.4 0.04}
\AddSpotColor{PANTONE} {PANTONE7509PC} {PANTONE\SpotSpace 7509\SpotSpace PC} {0 0.2 0.5 0.05}
\AddSpotColor{PANTONE} {PANTONE7510PC} {PANTONE\SpotSpace 7510\SpotSpace PC} {0 0.3 0.72 0.11}
\AddSpotColor{PANTONE} {PANTONE7511PC} {PANTONE\SpotSpace 7511\SpotSpace PC} {0 0.45 1 0.25}
\AddSpotColor{PANTONE} {PANTONE7512PC} {PANTONE\SpotSpace 7512\SpotSpace PC} {0 0.46 1 0.33}
\AddSpotColor{PANTONE} {PANTONE7513PC} {PANTONE\SpotSpace 7513\SpotSpace PC} {0 0.18 0.28 0.03}
\AddSpotColor{PANTONE} {PANTONE7514PC} {PANTONE\SpotSpace 7514\SpotSpace PC} {0 0.24 0.38 0.05}
\AddSpotColor{PANTONE} {PANTONE7515PC} {PANTONE\SpotSpace 7515\SpotSpace PC} {0 0.35 0.5 0.12}
\AddSpotColor{PANTONE} {PANTONE7516PC} {PANTONE\SpotSpace 7516\SpotSpace PC} {0 0.52 1 0.35}
\AddSpotColor{PANTONE} {PANTONE7517PC} {PANTONE\SpotSpace 7517\SpotSpace PC} {0 0.6 1 0.44}
\AddSpotColor{PANTONE} {PANTONE7518PC} {PANTONE\SpotSpace 7518\SpotSpace PC} {0 0.4 0.55 0.6}
\AddSpotColor{PANTONE} {PANTONE7519PC} {PANTONE\SpotSpace 7519\SpotSpace PC} {0.5 0.6 1 0.48}
\AddSpotColor{PANTONE} {PANTONE7520PC} {PANTONE\SpotSpace 7520\SpotSpace PC} {0 0.16 0.19 0}
\AddSpotColor{PANTONE} {PANTONE7521PC} {PANTONE\SpotSpace 7521\SpotSpace PC} {0 0.25 0.2 0.1}
\AddSpotColor{PANTONE} {PANTONE7522PC} {PANTONE\SpotSpace 7522\SpotSpace PC} {0 0.4 0.3 0.16}
\AddSpotColor{PANTONE} {PANTONE7523PC} {PANTONE\SpotSpace 7523\SpotSpace PC} {0 0.4 0.35 0.2}
\AddSpotColor{PANTONE} {PANTONE7524PC} {PANTONE\SpotSpace 7524\SpotSpace PC} {0 0.55 0.6 0.27}
\AddSpotColor{PANTONE} {PANTONE7525PC} {PANTONE\SpotSpace 7525\SpotSpace PC} {0 0.45 0.5 0.3}
\AddSpotColor{PANTONE} {PANTONE7526PC} {PANTONE\SpotSpace 7526\SpotSpace PC} {0 0.65 1 0.35}
\AddSpotColor{PANTONE} {PANTONE7527PC} {PANTONE\SpotSpace 7527\SpotSpace PC} {0 0.02 0.06 0.07}
\AddSpotColor{PANTONE} {PANTONE7528PC} {PANTONE\SpotSpace 7528\SpotSpace PC} {0 0.03 0.1 0.1}
\AddSpotColor{PANTONE} {PANTONE7529PC} {PANTONE\SpotSpace 7529\SpotSpace PC} {0 0.04 0.12 0.17}
\AddSpotColor{PANTONE} {PANTONE7530PC} {PANTONE\SpotSpace 7530\SpotSpace PC} {0 0.08 0.21 0.32}
\AddSpotColor{PANTONE} {PANTONE7531PC} {PANTONE\SpotSpace 7531\SpotSpace PC} {0 0.1 0.27 0.5}
\AddSpotColor{PANTONE} {PANTONE7532PC} {PANTONE\SpotSpace 7532\SpotSpace PC} {0 0.17 0.5 0.65}
\AddSpotColor{PANTONE} {PANTONE7533PC} {PANTONE\SpotSpace 7533\SpotSpace PC} {0 0.22 0.85 0.85}
\AddSpotColor{PANTONE} {PANTONE7534PC} {PANTONE\SpotSpace 7534\SpotSpace PC} {0 0.02 0.08 0.1}
\AddSpotColor{PANTONE} {PANTONE7535PC} {PANTONE\SpotSpace 7535\SpotSpace PC} {0 0.03 0.15 0.2}
\AddSpotColor{PANTONE} {PANTONE7536PC} {PANTONE\SpotSpace 7536\SpotSpace PC} {0 0.04 0.22 0.32}
\AddSpotColor{PANTONE} {PANTONE7537PC} {PANTONE\SpotSpace 7537\SpotSpace PC} {0.03 0 0.1 0.2}
\AddSpotColor{PANTONE} {PANTONE7538PC} {PANTONE\SpotSpace 7538\SpotSpace PC} {0.09 0 0.13 0.3}
\AddSpotColor{PANTONE} {PANTONE7539PC} {PANTONE\SpotSpace 7539\SpotSpace PC} {0.02 0 0.09 0.36}
\AddSpotColor{PANTONE} {PANTONE7540PC} {PANTONE\SpotSpace 7540\SpotSpace PC} {0 0 0 0.72}
\AddSpotColor{PANTONE} {PANTONE7541PC} {PANTONE\SpotSpace 7541\SpotSpace PC} {0.02 0 0 0.05}
\AddSpotColor{PANTONE} {PANTONE7542PC} {PANTONE\SpotSpace 7542\SpotSpace PC} {0.1 0 0.03 0.16}
\AddSpotColor{PANTONE} {PANTONE7543PC} {PANTONE\SpotSpace 7543\SpotSpace PC} {0.07 0 0 0.3}
\AddSpotColor{PANTONE} {PANTONE7544PC} {PANTONE\SpotSpace 7544\SpotSpace PC} {0.1 0.01 0 0.4}
\AddSpotColor{PANTONE} {PANTONE7545PC} {PANTONE\SpotSpace 7545\SpotSpace PC} {0.23 0.02 0 0.63}
\AddSpotColor{PANTONE} {PANTONE7546PC} {PANTONE\SpotSpace 7546\SpotSpace PC} {0.33 0.04 0 0.72}
\AddSpotColor{PANTONE} {PANTONE7547PC} {PANTONE\SpotSpace 7547\SpotSpace PC} {0.35 0.04 0 0.94}
\AddSpotColor{PANTONE} {PANTONEBlack2PC} {PANTONE\SpotSpace Black\SpotSpace 2\SpotSpace PC} {0 0.03 0.55 0.87}
\AddSpotColor{PANTONE} {PANTONEBlack3PC} {PANTONE\SpotSpace Black\SpotSpace 3\SpotSpace PC} {0.6 0 0.6 0.91}
\AddSpotColor{PANTONE} {PANTONEBlack4PC} {PANTONE\SpotSpace Black\SpotSpace 4\SpotSpace PC} {0 0.22 1 0.89}
\AddSpotColor{PANTONE} {PANTONEBlack5PC} {PANTONE\SpotSpace Black\SpotSpace 5\SpotSpace PC} {0 0.4 0.22 0.87}
\AddSpotColor{PANTONE} {PANTONEBlack6PC} {PANTONE\SpotSpace Black\SpotSpace 6\SpotSpace PC} {1 0.35 0 1}
\AddSpotColor{PANTONE} {PANTONEBlack7PC} {PANTONE\SpotSpace Black\SpotSpace 7\SpotSpace PC} {0 0 0.15 0.82}
\AddSpotColor{PANTONE} {PANTONEBlackPC} {PANTONE\SpotSpace Black\SpotSpace PC} {0 0.13 0.49 0.98}
\AddSpotColor{PANTONE} {PANTONEBlue072PC} {PANTONE\SpotSpace Blue\SpotSpace 072\SpotSpace PC} {1 0.88 0 0.05}
\AddSpotColor{PANTONE} {PANTONECoolGray1PC} {PANTONE\SpotSpace Cool\SpotSpace Gray\SpotSpace 1\SpotSpace PC} {0 0 0 0.06}
\AddSpotColor{PANTONE} {PANTONECoolGray2PC} {PANTONE\SpotSpace Cool\SpotSpace Gray\SpotSpace 2\SpotSpace PC} {0 0 0 0.1}
\AddSpotColor{PANTONE} {PANTONECoolGray3PC} {PANTONE\SpotSpace Cool\SpotSpace Gray\SpotSpace 3\SpotSpace PC} {0 0 0 0.17}
\AddSpotColor{PANTONE} {PANTONECoolGray4PC} {PANTONE\SpotSpace Cool\SpotSpace Gray\SpotSpace 4\SpotSpace PC} {0 0 0 0.24}
\AddSpotColor{PANTONE} {PANTONECoolGray5PC} {PANTONE\SpotSpace Cool\SpotSpace Gray\SpotSpace 5\SpotSpace PC} {0 0 0 0.29}
\AddSpotColor{PANTONE} {PANTONECoolGray6PC} {PANTONE\SpotSpace Cool\SpotSpace Gray\SpotSpace 6\SpotSpace PC} {0 0 0 0.31}
\AddSpotColor{PANTONE} {PANTONECoolGray7PC} {PANTONE\SpotSpace Cool\SpotSpace Gray\SpotSpace 7\SpotSpace PC} {0 0 0 0.37}
\AddSpotColor{PANTONE} {PANTONECoolGray8PC} {PANTONE\SpotSpace Cool\SpotSpace Gray\SpotSpace 8\SpotSpace PC} {0 0.01 0 0.43}
\AddSpotColor{PANTONE} {PANTONECoolGray9PC} {PANTONE\SpotSpace Cool\SpotSpace Gray\SpotSpace 9\SpotSpace PC} {0 0.01 0 0.51}
\AddSpotColor{PANTONE} {PANTONECoolGray10PC} {PANTONE\SpotSpace Cool\SpotSpace Gray\SpotSpace 10\SpotSpace PC} {0 0.02 0 0.6}
\AddSpotColor{PANTONE} {PANTONECoolGray11PC} {PANTONE\SpotSpace Cool\SpotSpace Gray\SpotSpace 11\SpotSpace PC} {0 0.02 0 0.68}
\AddSpotColor{PANTONE} {PANTONEGreenPC} {PANTONE\SpotSpace Green\SpotSpace PC} {1 0 0.59 0}
\AddSpotColor{PANTONE} {PANTONEOrange021PC} {PANTONE\SpotSpace Orange\SpotSpace 021\SpotSpace PC} {0 0.53 1 0}
\AddSpotColor{PANTONE} {PANTONEProc.BlackPC} {PANTONE\SpotSpace Proc.\SpotSpace Black\SpotSpace PC} {0 0 0 1}
\AddSpotColor{PANTONE} {PANTONEProc.BluePC} {PANTONE\SpotSpace Proc.\SpotSpace Blue\SpotSpace PC} {1 0.1 0 0.1}
\AddSpotColor{PANTONE} {PANTONEProc.CyanPC} {PANTONE\SpotSpace Proc.\SpotSpace Cyan\SpotSpace PC} {1 0 0 0}
\AddSpotColor{PANTONE} {PANTONEProc.Magen.PC} {PANTONE\SpotSpace Proc.\SpotSpace Magen.\SpotSpace PC} {0 1 0 0}
\AddSpotColor{PANTONE} {PANTONEProc.YellowPC} {PANTONE\SpotSpace Proc.\SpotSpace Yellow\SpotSpace PC} {0 0 1 0}
\AddSpotColor{PANTONE} {PANTONEPurplePC} {PANTONE\SpotSpace Purple\SpotSpace PC} {0.38 0.88 0 0}
\AddSpotColor{PANTONE} {PANTONERed032PC} {PANTONE\SpotSpace Red\SpotSpace 032\SpotSpace PC} {0 0.9 0.86 0}
\AddSpotColor{PANTONE} {PANTONERef.BluePC} {PANTONE\SpotSpace Ref.\SpotSpace Blue\SpotSpace PC} {1 0.73 0 0.02}
\AddSpotColor{PANTONE} {PANTONERhod.RedPC} {PANTONE\SpotSpace Rhod.\SpotSpace Red\SpotSpace PC} {0.03 0.89 0 0}
\AddSpotColor{PANTONE} {PANTONERub.RedPC} {PANTONE\SpotSpace Rub.\SpotSpace Red\SpotSpace PC} {0 1 0.15 0.04}
\AddSpotColor{PANTONE} {PANTONEVioletPC} {PANTONE\SpotSpace Violet\SpotSpace PC} {0.98 1 0 0}
\AddSpotColor{PANTONE} {PANTONEWarmGray1PC} {PANTONE\SpotSpace Warm\SpotSpace Gray\SpotSpace 1\SpotSpace PC} {0 0.02 0.03 0.06}
\AddSpotColor{PANTONE} {PANTONEWarmGray2PC} {PANTONE\SpotSpace Warm\SpotSpace Gray\SpotSpace 2\SpotSpace PC} {0 0.02 0.05 0.09}
\AddSpotColor{PANTONE} {PANTONEWarmGray3PC} {PANTONE\SpotSpace Warm\SpotSpace Gray\SpotSpace 3\SpotSpace PC} {0 0.04 0.08 0.17}
\AddSpotColor{PANTONE} {PANTONEWarmGray4PC} {PANTONE\SpotSpace Warm\SpotSpace Gray\SpotSpace 4\SpotSpace PC} {0 0.04 0.09 0.24}
\AddSpotColor{PANTONE} {PANTONEWarmGray5PC} {PANTONE\SpotSpace Warm\SpotSpace Gray\SpotSpace 5\SpotSpace PC} {0 0.05 0.1 0.29}
\AddSpotColor{PANTONE} {PANTONEWarmGray6PC} {PANTONE\SpotSpace Warm\SpotSpace Gray\SpotSpace 6\SpotSpace PC} {0 0.06 0.12 0.31}
\AddSpotColor{PANTONE} {PANTONEWarmGray7PC} {PANTONE\SpotSpace Warm\SpotSpace Gray\SpotSpace 7\SpotSpace PC} {0 0.08 0.14 0.38}
\AddSpotColor{PANTONE} {PANTONEWarmGray8PC} {PANTONE\SpotSpace Warm\SpotSpace Gray\SpotSpace 8\SpotSpace PC} {0 0.09 0.16 0.43}
\AddSpotColor{PANTONE} {PANTONEWarmGray9PC} {PANTONE\SpotSpace Warm\SpotSpace Gray\SpotSpace 9\SpotSpace PC} {0 0.11 0.2 0.47}
\AddSpotColor{PANTONE} {PANTONEWarmGray10PC} {PANTONE\SpotSpace Warm\SpotSpace Gray\SpotSpace 10\SpotSpace PC} {0 0.14 0.28 0.55}
\AddSpotColor{PANTONE} {PANTONEWarmGray11PC} {PANTONE\SpotSpace Warm\SpotSpace Gray\SpotSpace 11\SpotSpace PC} {0 0.17 0.34 0.62}
\AddSpotColor{PANTONE} {PANTONEWarmRedPC} {PANTONE\SpotSpace Warm\SpotSpace Red\SpotSpace PC} {0 0.75 0.9 0}
\AddSpotColor{PANTONE} {PANTONEYellowPC} {PANTONE\SpotSpace Yellow\SpotSpace PC} {0 0.01 1 0}


==> subfloat/Makefile <==
SUBFLOATDIR=subfloat
INSTALLDIR=`kpsewhich --expand-path='$$TEXMFLOCAL'`/tex/latex/subfloat
DOCDIR=`kpsewhich --expand-path='$$TEXMFLOCAL'`/doc/latex/subfloat
VERSION=`grep '^\\\\def\\\\fileversion' subfloat.dtx | sed 's/^\\\\def\\\\fileversion{\\(.*\\)\\.\\(.*\\)}/\\1_\\2/'`

.SUFFIXES: .sty .ins .dtx .dvi .ps


.ins.sty:
	latex $<

.dtx.dvi:
	latex $<
	latex $<
	makeindex -s gind.ist $(*D)/$(*F)
	makeindex -s gglo.ist -o $(*D)/$(*F).gls $(*D)/$(*F).glo
	latex $<

.dvi.ps:
	dvips -o $(*D)/$(*F).ps $(*D)/$(*F)


all: subfloat.sty subfloat.dvi ausgabe 

subfloat: subfloat.sty

clean:
	@-rm -f subfloat.{glo,gls,idx,ilg,ind,aux,log,toc}
	@-rm -f *~

distclean: clean
	@-rm -f subfloat.{sty,dvi,ps}

tar:	all clean
	echo Lege subfloat.tar.gz an
	-rm -f subfloat-*.tar.gz
	tar czCf .. subfloat-$(VERSION).tar.gz \
	  $(SUBFLOATDIR)/README $(SUBFLOATDIR)/Makefile \
	  $(SUBFLOATDIR)/subfloat.{dtx,ins,dvi} \
	  $(SUBFLOATDIR)/install.sh \
	  $(SUBFLOATDIR)/subfloat.xml $(SUBFLOATDIR)/ChangeLog

zip:	all clean
	-@rm -f subfloat-$(VERSION).zip
	mkdirhier tex/latex/subfloat
	mkdirhier doc/latex/subfloat
	mkdirhier source/latex/subfloat
	mv subfloat.sty tex/latex/subfloat
	cp subfloat.{dtx,ins,xml} Makefile source/latex/subfloat
	cp ChangeLog README subfloat.dvi doc/latex/subfloat
	zip -r subfloat-$(VERSION).zip tex doc source
	rm -r tex/ doc/ source/

install: all
	if [ ! -d $(INSTALLDIR) ]; then mkdirhier $(INSTALLDIR); fi
	if [ ! -d $(DOCDIR) ]; then mkdirhier $(DOCDIR); fi
	install -m622 subfloat.sty $(INSTALLDIR)
	install -m622 subfloat.dvi $(DOCDIR)
	texhash

ausgabe:
	@echo "Please copy subfloat.sty to a directory"
	@echo "in the LaTeX search path"

tpm:	all
	mkdirhier texmf-local/tex/latex/subfloat
	mkdirhier texmf-local/doc/latex/subfloat
	mkdirhier texmf-local/source/latex/subfloat
	cp subfloat.dtx subfloat.ins README Makefile texmf-local/source/latex/subfloat
	cp README subfloat.dvi texmf-local/doc/latex/subfloat
	cp subfloat.sty texmf-local/tex/latex/subfloat
	@-rm -f subfloat.zip
	zip -r subfloat texmf-local
	rm -rf texmf-local



subfloat.sty: subfloat.ins subfloat.dtx



